Smart-PGSim: Using Neural Network to Accelerate AC-OPF Power Grid Simulation

The optimal power flow (OPF) problem is one of the most important optimization problems for the operation of the power grid. It calculates the optimum scheduling of the committed generation units. In this paper, we develop a neural network approach to the problem of accelerating the current optimal power flow (AC-OPF) by generating an intelligent initial solution. The high quality of the initial solution and guidance of other outputs generated by the neural network enables faster convergence to the solution without losing optimality of final solution as computed by traditional methods. Smart-PGSim generates a novel multitask-learning neural network model to accelerate the AC-OPF simulation. Smart-PGSim also imposes the physical constraints of the simulation on the neural network automatically. Smart-PGSim brings an average of 49.2% performance improvement (up to 91%), computed over 10,000 problem simulations, with respect to the original AC-OPF implementation, without losing the optimality of the final solution.

==> Content/ModelEvolution.tex <==
\subsection{Sensitivity analysis --- Prior}
\label{sec4-3}

After the analysis of the success rate, it is crucial to design an efficient neural network model for the AC-OPF problem. Once the model is ready, we can use a neural network model to generate simulation outputs as a good initial point of MIPS to accelerate simulation convergence. 
However, there is no systematic way to design the topology of neural network models for accelerating HPC applications~\cite{baker2018brochure}.
Based on the component study in Section~\ref{sec5-1:com_ana}, variable sensitivity is crucial for simulation convergence and acceleration. 
We involve variable sensitivity to guide our model design. 
Here, we define variable sensitivity as to how much extent the variation of output precision impacts the simulation convergence and acceleration. 
Through involving the variable sensitivity, it is efficient to guide the network morphism~\cite{wei2016network} during model construction. 

However, there are several challenges. 
Through component study, we observe that variables sensitivity is difficult to be quantified.
Simulation convergence and acceleration varies with the precision of multiple variables.
But, we are not of aware which or what combinations of these variables are most critical to the problem solution.
It is hard to map the variance of variable precision to the fluctuation of speedup.
Also, the training overhead for model validation is expensive because, during the search, each evaluation of a morphism direction involves intensive computation for training and testing the neural network model.

To address these challenges, we propose a quality-prior mechanism to explore the morphism direction based on sensitivity results automatically. 
Our algorithm is listed in Algorithm~\ref{alg:morph}.
We empirically design a basic model $G$ based on our domain knowledge and evolve the basic model in the following morphism iterations until the model satisfies the user's requirement.
In a morphism iteration, we first generate model outputs and calculate the output loss (Line 3-4).
We define the output loss using Mean Absolute Percentage Error (MAPE), i.e., the difference of each element between model outputs and the ground-truth:
\begin{equation}
    MAPE(x) =\frac{100\%}{n} \sum_{i=1}^{n}\left|\frac{x_i-gt_i}{gt_i+\epsilon}\right|%(x_i\in x)
\end{equation}
This is a quantitative measurement of variable precision. We set the $\epsilon$ as $e-9$ in case of $gt_i=0$.


Then, we perform a prior analysis (Line 5-9).
We generate multiple prior cases, including all output variables of model $G$ and each variable in the prior case combining two precise levels, i.e., keep the current precision or improve the variable precision (Line 6). 
We use the ground-truth value to improve variable precision (Line 7). Through choosing the precise level, there can be as many as $2^n$ prior cases ($n$ is the number of variables). %For example, there are 16 prior cases for $X, \lambda, \mu, Z$ in our paper.
\textcolor{wq}{In this paper, we have 16 prior cases by choosing the precise levels of variables $X, \lambda, \mu, Z$.}
We adopt the MIPS to collect the speedup results of all prior cases (Line 8).
After analyzing the obtained results, we select the best prior case, i.e., the case with the highest speedup (Line 9).
Comparing a exhausted search, the prior analysis is light-weighted and significantly mitigates the training overhead of inefficient models during evolution. 
\textcolor{review}{Review4:(1) For example, Alg 1 on Prior analysis is not clear at all, what does the “precise level” mean? What does D\_gt in line 7 mean? How would deep(G, u0) and wide (G, U0, p) work with the multi-task learning framework? Are they only used for the shared network? (2) The paper has a few places to measure the difference between prediction and ground truth, but each one uses a different flavor of metrics to measure the differences, see (8), (10), (17). It’s not clear why it should be so and the justification?}

Based on the best prior case, we introduce two morphism operations to evolve Model $G$ (Line 11), 
i.e., $deep(G, u0)$ and $wide(G, U_0, p)$. 
Operation $deep(G, u_0)$ is adding a layer after layer $u_0$. We insert a layer with the same topology as $u_0$ in our paper to implement the operation. 
Operation $wide(G, u_0, p)$ is widening the layer $u_0$ with a specific proportion (i.e., $10\%$ in our paper).
After the evolution, we retrain the model (Line 12) until it is ready to generate the solution to simulation.
\begin{algorithm}%[!t] 
\caption{Quality-prior Model Morphism}
\label{alg:morph}
\begin{algorithmic}[1]
 \REQUIRE A basic neural network model $G$; Ground truth data $D_{gt}$;  
 \STATE Start with a basic model $G$\\
 \STATE  \textbf{do}
 \bdwqindent
    \STATE Fetch model outputs $T = \{ T_1, ... , T_n\}$
    \STATE Calculate and collect the loss on each output, i.e., $MAPE(T)=\{MAPE(T_1), ..., MAPE(T_n)\}$ ($n$ is the number of variables); 
    \STATE \textbf{Prior analysis:}
    \bwqindent
    \STATE Generate $2^n$ different prior cases;
   \STATE Use $D_{gt}$ to decrease the loss of outputs $MAPE(T)$;  
   \STATE Collect performance results of prior cases in MIPS;
   \STATE Record the best prior case;
    \ewqindent
    \STATE \textbf{Model morphism:}
    \bwqindent
   \STATE  Evolve model $G$ by $deep(G, u0)$ or $wide(G, U_0, p)$;
   \STATE  Re-train model $G$; 
    \ewqindent
   \edwqindent
 \STATE \textbf{while} Loss of model $G$ reaches user's requirement
\RETURN $G$ 
\end{algorithmic}
\end{algorithm}

==> Content/draft.tex <==

\begin{comment}
\textcolor{gokcen}{We need to give a little bit more details here or we risk to raise more questions than we answer. Currently, it's not very clear what we have done and the parallelization strategy we followed. In general, scaling should be simple: the problem is embarrassingly parallel (each scenario can be evaluated independently) thus we divide the scenarios among the distributed compute nodes first and then, within each node, we divide the scenarios among GPUs (inference + MIPS). During training, we can follow the data parallel model. I would imagine reviewers would mostly be interested in the former. }
\textcolor{wq}{Yes, the current experiments is following the former one. We distribute the input problems (scenarios) to multiple nodes.  I didn't show anything for training. (because we don't want to emphasis the high overhead in NN training).} 
I have several questions and comments. 1. if we talk about multi-node, reviewers will expect a cluster of compute nodes interconnected through some form of high-performance network and that our model uses something like MPI. How many nodes do we have? how many GPUs/node? 
\textcolor{wq}{In total, we have 128GPUs. In particular, we 16 DGX-1 nodes and each DGX-1 node has 8 GPUs. }
\textcolor{gokcen}{
2. How do we run each scenario? Is the data in fig 9 for inference or training? At high level we have two combined tasks (ML running on GPU and MIPS running on CPU). Both GPU and CPU can run multiple scenarios at the same time. Are we submitting multiple inferences to a single GPU at the same time? if so, how do we link to the corresponding MIPS part and keep track of what scenarios we have executed? }
\textcolor{wq}{Fig. 9 is for inference. Between nodes, we distribute scenarios manually (there are no extra data copy overhead). Inside the node, the NN model and input data are allocated on device[0] and then device[0] copy the NN model and distribute the input data to other 7 GPUs. I didn't test the execution time in MIPS. This is a very good point that ML running on GPU and MIPS running on CPU, but Matpower can not be run parallel on CPUs. If we follow the above idea, which means we have two CPUs work for MIPS sequentially (executed one by one) in each node, this process will be super slow (around 1000x longer than NN inference) and we may have no reason to use multiple GPUs for inference.   }
\textcolor{gokcen}{3. strong scaling means that the number of scenarios is fixed or the bus size? weak scaling means that the number of scenarios increases with the number of compute nodes/GPUs? }
\textcolor{wq}{strong scaling means that the number of scenarios is fixed. weak scaling means that the number of scenarios increases with the number of compute nodes/GPUs. }
\textcolor{gokcen}{4. If the problem is embarrassingly parallel, why don't we see close-to-linear speedup in fig 9? }
\textcolor{wq}{Inside the node, we still have overhead of data copy. we will upload all data to Device[0], and device[0] is charged for copying the NN model and distributing the input data to other 7 GPUs. This is implemented by the  pytorch function DataParallel().} \url{https://pytorch.org/tutorials/beginner/blitz/data_parallel_tutorial.html}
\textcolor{gokcen}{5. how is device[0] distributing work to the other devices? are we using GPU-RDMA over NVLINK? what about the MIPS part?}
\textcolor{wq}{Inside the GPUs, we copy data using NVLINK. I do not have the answer for MIPS now. Previously, we manually copy the data.}
\end{comment}

% \begin{table}[]
% \begin{adjustbox}{width=1.0\linewidth}
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% \multirow{3}{*}{\textbf{Ahmed's model}}            & \textbf{Test system} & --              & \textbf{39-bus} & \textbf{57-bus} & \textbf{118-bus} & \textbf{--}      \\ \cline{2-7} 
%                                                   & \textbf{SF}          & --              & $15.38\times$   & $9.49\times$    & $7.97\times$     & --               \\ \cline{2-7} 
%                                                   & \textbf{$L_{cost}$}  & --              & $0.326\%$       & $0.457\%$       & $0.821\%$        & --               \\ \hline
% \multirow{3}{*}{\textbf{\name}} & \textbf{Test system} & \textbf{14-bus} & \textbf{30-bus} & \textbf{57-bus} & \textbf{118-bus} & \textbf{300-bus} \\ \cline{2-7} 
%                                                   & \textbf{SF}          & $21.17\times$   & $40.19\times$   & $21.72\times$   & $36.15\times$    & $105.64\times$   \\ \cline{2-7} 
%                                                   & \textbf{$L_{cost}$}  & $0.007\%$       & $0.074\%$       & $0.040\%$       & $0.003\%$        & $0.008\%$        \\ \hline
% \end{tabular}
% \end{adjustbox}
% \end{table}

%\noindent\textbf{Time Comparison.} 

%\noindent\textbf{Avg. Cost Deviation.} 
%\vspace{5pt}

% Figure~\ref{fig:sec7_1} shows the results for \name with different system sizes. The bar shows the speedup comparing with the MIPS solver. 
% In all test systems, \name significantly outperforms the MIPS solver and achieves $45.0\times$ speedup on average.
% Even with the increased size of the power network size, our model provides considerable performance gain.
% The largest improvement over MIPS solver is $105.6\times$ on the 300-bus test system.

% Besides the execution time, we also study the simulation quality of \name. 
% We use 10,000 input problems to evaluate each test system. 
% We take the final solution of MIPS as the ground truth and study the quality loss of the model prediction. 
% The ``*'' markers indicate the cost deviation $L_{cost}$ to show the results of the quality loss for all input problems with five selected grid sizes. 
% We observe that \name consistently achieves good accuracy on different test systems, and all losses are under $0.1\%$.
\subsection{Comparison with Prior Work}
% \begin{figure}[!t]
%   \centering
%   \includegraphics[width=1.0\linewidth]{Figures/sec7_1.pdf}
%   \caption{Performance of \name}
%   \label{fig:sec7_1} 
% \end{figure}

To fairly compare with the state-of-the-art method, i.e., Ahmed's model, we directly take the prediction of \name as final solution. We compare the performance of the execution time and the optimality loss which used in  Ahmed's model.
%We first directly use \name to replace the entire solving process in MIPS and test the performance of . 
%when the output of \name is used as a warm-start point to solve the AC-OPF problem.
%\textcolor{gk}{I am a little confused here a little, in this sub-section, we replace the entire computation with the NN model, so why do we start the sentence with "warm-start"?}
%We take the MIPS solver as the baseline method. MIPS is the traditional method used in the Matpower and does not include any neural network.
%Compared with neural network-based acceleration, MIPS has the highest simulation quality, but the performance is limited. All performance (execution time) reported in this section is shown as ``speedup'' concerning the performance of MIPS.
%\textcolor{review}{Review4:Directly using the predicted solutions of neural networks will cause a wrong solution and may not be accepted as a physical solution.}
%We involve two factors here to measure the performance.
Time comparison shows the speedup of using a neural network to replace the whole solving process of MIPS. Cost deviation measures simulation quality. We donate a speedup factor (SF) to measure the computational improvements: $SF = \frac{1}{n}\sum_{i=1}^{n} {(T^{MTL}_{i}}/{T^{MIPS}_{i})}, $ where $T^{MTL}_i$ refers the execution time of the multi-task model and $T^{MIPS}_i$ represents the execution time of the numerical solver (MIPS) for each input problem $i$.
We measure the loss using the average fractional difference between the cost of predicted solution and the cost of the true solution:
$L_{cost} = \frac{100\%}{n} \sum_{i=1}^{n}\left|1-\frac{pred cost_{i}}{true cost{i}}\right|$.
Observed from Table~\ref{tab:model_perf}, our framework \name outperforms the state of the art model (Ahmed's model). \name achieves an average $44.97\times$ speedup which provides $330\%$ improvement comparing the average speedup of Ahmed's model ($32.84\%$). Meanwhile, \name decrease the cost loss $12.16\times$ by average comparing with Ahmed's model.


\begin{table}
\normalsize
\caption{Prediction Performance Comparison.} 
\label{tab:model_perf}
\begin{adjustbox}{width=1.0\linewidth}
\begin{tabular}{c cccccc}
%\footnotesize
\toprule 
\multirow{3}{*}[-0.33em]{\textbf{Ahmed's model}}            & \textbf{Test system} & --              & \textbf{39-bus} & \textbf{57-bus} & \textbf{118-bus} & \textbf{--} \\
\cmidrule(lr){2-7}
& \textbf{SF }& -- & $15.38\times$ &$9.49\times$ & $7.97\times$& --\\
&\textbf{$L_{cost}$}& -- & $0.326\%$ & $0.457\%$& $0.821\%$& -- \\
\midrule
\multirow{3}{*}[-0.33em]{\textbf{\name}} & \textbf{Test system} & \textbf{14-bus} & \textbf{30-bus} & \textbf{57-bus} & \textbf{118-bus} & \textbf{300-bus} \\
\cmidrule(lr){2-7}
&\textbf{SF} & $21.17\times$  & $40.19\times$ &$21.72\times$ & $36.15\times$& $105.64\times$ \\
&\textbf{$L_{cost}$}& $0.007\%$ & $0.074\%$ & $0.040\%$& $0.003\%$& $0.008\%$ \\

% \cmidrule(lr){2-7}
% Ahmed& -- & 39-bus & 57-bus & 118-bus & -- \\
% SF & -- & $15.38\times$ &$9.49\times$ & $7.97\times$& --\\
% $L_{cost}$& -- & $0.326\%$ & $0.457\%$& $0.821\%$& -- \\
% 
% & 14-bus & 30-bus & 57-bus & 118-bus & 300-bus \\
% SF & $21.17\times$  & $40.19\times$ &$21.72\times$ & $36.15\times$& $105.64\times$ \\
% $L_{cost}$& $0.007\%$ & $0.074\%$ & $0.040\%$& $0.003\%$& $0.008\%$ \\
 \bottomrule
\end{tabular}
\end{adjustbox}
\end{table}


% \begin{table}[]
% \begin{adjustbox}{width=1.0\linewidth}
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% \multirow{3}{*}{\textbf{Ahmed's model}}            & \textbf{Test system} & --              & \textbf{39-bus} & \textbf{57-bus} & \textbf{118-bus} & \textbf{--}      \\ \cline{2-7} 
%                                                   & \textbf{SF}          & --              & $15.38\times$   & $9.49\times$    & $7.97\times$     & --               \\ \cline{2-7} 
%                                                   & \textbf{$L_{cost}$}  & --              & $0.326\%$       & $0.457\%$       & $0.821\%$        & --               \\ \hline
% \multirow{3}{*}{\textbf{\name}} & \textbf{Test system} & \textbf{14-bus} & \textbf{30-bus} & \textbf{57-bus} & \textbf{118-bus} & \textbf{300-bus} \\ \cline{2-7} 
%                                                   & \textbf{SF}          & $21.17\times$   & $40.19\times$   & $21.72\times$   & $36.15\times$    & $105.64\times$   \\ \cline{2-7} 
%                                                   & \textbf{$L_{cost}$}  & $0.007\%$       & $0.074\%$       & $0.040\%$       & $0.003\%$        & $0.008\%$        \\ \hline
% \end{tabular}
% \end{adjustbox}
% \end{table}

%\noindent\textbf{Time Comparison.} 

%\noindent\textbf{Avg. Cost Deviation.} 
%\vspace{5pt}

% Figure~\ref{fig:sec7_1} shows the results for \name with different system sizes. The bar shows the speedup comparing with the MIPS solver. 
% In all test systems, \name significantly outperforms the MIPS solver and achieves $45.0\times$ speedup on average.
% Even with the increased size of the power network size, our model provides considerable performance gain.
% The largest improvement over MIPS solver is $105.6\times$ on the 300-bus test system.

% Besides the execution time, we also study the simulation quality of \name. 
% We use 10,000 input problems to evaluate each test system. 
% We take the final solution of MIPS as the ground truth and study the quality loss of the model prediction. 
% The ``*'' markers indicate the cost deviation $L_{cost}$ to show the results of the quality loss for all input problems with five selected grid sizes. 
% We observe that \name consistently achieves good accuracy on different test systems, and all losses are under $0.1\%$.


%\textcolor{gokcen}{It might be better to describe briefly what \name is, (because we pass two sections after intro, readers might need to be reminded what the paper is about, then we can say this section overviews \name)}
%\textcolor{wq}{We develop a framework \name, a novel multitask-learning  neural network model incorporating physical constraints to accelerate the AC-OPF simulation.}
%We overview our proposed framework ``\name" in this section. 


%Alternating current optimal power flow (AC-OPF) problem is critical to power grid operations. In this paper, we develop a neural network (NN)-based approach to accelerate the solving process of AC-OPF by generating an intelligent initial solution. The high quality of the initial solution and guidance of other outputs from NN enable faster computation convergence without losing solution optimality. We develop a framework,  \name. \name generates an NN model that uses variables critical to the problem convergence as a part of the model output, and includes a tool to quantify the sensitivity of simulation time and convergence to the variables. \name generates a novel multitask-learning NN model which allows information sharing when predicting multiple variables, while including customized layers to predict individual variables. \name also imposes physical constraints from AC-OPF on NN.  \name brings $2.60\times$ speedup on average (up to $3.28\times$) computed over 10,000 problems, without losing solution optimality.% \textcolor{dong}{150 words now}
%Third, how to impose physical constraints on NN to ensure the validness of NN prediction. % is a challenge. 
%Traditionally, the NN model is manually constructed by computer scientists as a black box with limited or no domain knowledge and without considering domain requirements. However, the AC-OPF problem has a set of physical constraints, such as power generation constraints, line flow constraints, and bus voltage constraints. Incorporating these physical constraints into our model not only increases the efficiency of NN model but also increase the quality of the final solution.

%\textcolor{blue}{% is a challenge. %Instead of shifting to trust in the correctness of such data mining algorithms, %\name evaluates variables critical to the simulation convergence to determine features for model training. In particular, \name checks the convergence criteria in the MatPower code to find those variables directly involved into the computation of determining if the simulation is converged. 
%Observations 1 and 4 indicates that our model design should target on multi-task prediction and consider feature dependency.%Multi-task prediction means the NN model should be constructed to generate multiple variables as output\textcolor{zhen}{wrong description}. %\textcolor{gokcen}{it might be better to put a reference here for these for conditions, even matpower reference}.
%The Newton Method involves large computation overhead; In each iteration of the Newton method, the Newton update happens. The Newton update is taken as follows: (1) update $ X$ and $\lambda$; (2) update $Z$ based on $ X$; and (3) update $\mu$ based on $X$ and $ Z$. %Different from the existing efforts, we incorporate a neural network model with physical constraints to address the limitation of flexibility and generality of the machine learning model and reduce computing overhead significantly %\textcolor{gokcen}{while obtaining feasible solutions.}

% \textcolor{red}{(This paragraph introduces a lot of background on multitask learning, which is overlapping with Section IV.A. We should simplify this paragraph.) }
% Multitask learning~\cite{battaglia2018relational, hand2017attributes} aims to simultaneously obtain the inference results for multiple tasks, \textcolor{dong}{which otherwise have to be solved with multiple neural network models. }
% %that are used to be solved separately with different neural network models.
% Multitask learning models are typically composed of shared layers and task-specific layers.  The shared layers are responsible for extracting common features for various tasks while the task-specific layer borrows the information from those common features to generate their dedicated results. Compared to use one model per task, the multi-task learning mechanism uses one model for multiple tasks by reducing model parameters via weight-sharing. Furthermore, multitask learning helps reduce the inductive bias that may occur in each  task~\cite{caruana1997multitask}.  For example, Ranjan~et al.~\cite{Ranjan2019HyperFace} propose a multitask model for face detection, landmarks localization, pose estimation, and gender recognition. In natural language processing,  Collobert et al.~\cite{collobert2008unified} develop a single language model that learns common latent features and combines multiple language processing predictions to improve prediction accuracy. 
% In this work, we use \textcolor{dong}{a physical constraint-based multitask model}  to take full advantage of the connections between those potentially relevant outputs. %and generates a precise warm-start point to reduce the number of subsequent iterations.
%This section overviews the proposed framework ``\name".
%Figure~\ref{fig:overview} shows the workflow of \name. The workflow includes two phases: offline and online phases. The offline phase is used to generate training data and determine \textcolor{zhen}{the most crucial} features \textcolor{zhen}{that can be predicted} by \textcolor{zhen}{\sout{build}} a NN-based \textcolor{zhen}{\sout{prediction}} model. \textcolor{zhen}{\sout{To collect training data}So in order to select key features and build this model}, \name injects various input problems (power loads) into MIPS \textcolor{zhen}{followed by a sensitivity study}, and then collects simulation results \textcolor{zhen}{as training data}. A pair of an input problem and the corresponding simulation result forms a training sample.%\textcolor{zhen}{\sout{To determine features (in other words, determining variables in MIPS as the output of the prediction model) and guide the NN model design, \name uses \textit{sensitivity study}  (Section~\ref{sec:sensi_study}).  
%Sensitivity study identifies the most important features and quantifies the impact of the noisy variables (i.e., the variables with some accuracy loss) on simulation success and performance (execution time). The results in sensitivity study are used to guide the topology design of NN model.}}%The user applies the model to generate a warm-start solution for MIPS (or other numerical solvers) to quickly converge.
\begin{comment}
The optimal power flow (OPF) problem is one of the most important optimization problems for the operation of the power grid that calculates the optimum scheduling of the committed generation units.
Power grid operators repeatedly solve the OPF problem multiple times per minute every day of the year, for decades, to ensure that the power grid system is operating reliably and safely. 
Provisioning, optimizing, and operating the power grid is a mission- and time-critical problem that involves complex simulations with high requirements and low latency.
In this paper, we develop a neural network approach to accelerate current optimal power flow (AC-OPF) problem solution by generating an intelligent initial solution.
The high quality of the initial solution and guidance of other outputs generated by the neural network enables the faster convergence to the solution without losing the optimality of the final solution as computed by traditional methods.
We develop a framework, called \name, that facilitates the construction of the neural network. 
\name generates the neural network model that uses variables critical for the problem convergence as a part of the model output, and includes a tool to quantify the sensitivity of simulation execution time and convergence to those variables. 
\name generates a novel multitask-learning neural network model to accelerate the AC-OPF simulation. 
The model topology allows information sharing when predicting multiple variables, while including customized layers to predict individual variables. 
\name also imposes the physical constraints of the simulation on the neural network automatically.  
 \name brings an average of 49.2\% performance improvement (and up to 91\%) computed over 10,000 problem simulations with respect to the original AC-OPF implementation, without losing the optimality of the final solution. 
\end{comment} %and the overhead of multiple models in which each .% The noise brought by sharing can improve model generalization. Parameter sharing is also helpful to reduce computation overhead suffered by using multiple separate models without parameter sharing.%The interaction between different tasks effectively helps the model escaping from the local minimum.

\begin{comment}
Based on observation 1, precise $X$ guarantees the success simulation convergence while Lagrangian factors $\lambda$, $\mu$, and $Z$ assist for simulation acceleration.
We prioritize feature by introducing the main task and auxiliary task. Main task is the optimization vector $X$ in Eqn.~\ref{eq:xvariable}, which provides the solution for the AC-OPF problem.
Auxiliary tasks are the Lagrangian factors (i.e., $\lambda$, $\mu$, and $z$). We estimate $\lambda$, $\mu$ and $z$ as an augmentation to provide additional information for main tasks. Through ``eavesdropping'' the auxiliary tasks, the main tasks interact with relevant tasks implicitly. 
 %The optimization vector (or the optimization variable) $X$ includes voltage angles $V_a$,  magnitudes $V_m$, generator active injections $P_g$ and reactive power injections $Q_g$.%In auxiliary tasks, we apply ``detach()" method to disables automatic differentiation, i.e stops keeping track of gradients in model training.
\end{comment}

%We aim to learn the direct solution $X$ in the main task to guarantee simulation quantity while estimating the Lagrangian factors $\lambda$, $\mu$, and $Z$ in the auxiliary tasks to maximize the speedup performance.
%\textbf{Enforcing prediction order. }
%\textcolor{gokcen}%\textcolor{red}{(double check if the above discussion is correct.)}
% \textcolor{gokcen}{I think we need a better justification, how we found this ordering among these features. Observation 2 and 3 don't justify the ordering described above. Can we refer to any equations that we used before? }\textcolor{wq}{wq: there are complicated equations and no space to involve them in the background section. I add two refs to show the justification. }

%From observation 2, Lagrangian factor $\lambda$ is independent while $Z$ is reply on $\mu$. To maximize the benefit of information sharing, we consider take a hierarchy for forecasting according to the physics dependency. We further check computational flow in MIPS, the solving process takes the order of (1) computing $X$ and $\lambda$; (2) computing $Z$ based on $X$; and (3) computing $\mu$ based on $X$ and $Z$. The computation dependency validates sensitivity observation and provide guide for prediction hierarchy.   

% The computation order show a strong dependency between these tasks, which is also validated in Observation 1 and Observation 2 of Section~\ref{sec:sensi_study}. 
% As shown in Figure~\ref{fig:MTL}, we take the computation order as the forecasting hierarchy in multitask learning model.

%\textcolor{dong}{
% \textcolor{dong}{%{especially for the Matpower-based power grid simulation and }%\textcolor{dong}{The observations 2 and 3 reveal the independence of $\lambda$ and the dependence of $Z$ on $\mu$. }%\textcolor{red}{(how did we predict $Z$?) }}
%\textcolor{red}{(Please double check if the above discussion is correct)}

% \textcolor{gokcen}{
%  Also, this description above doesn't completely follow the figure 2. Figure 2 shows that we calculate Z, then $\mu$ from Z.
%  }
 
%take a hierarchy for forecasting according to the physics dependency. First, we infer the main task $X$($V_a$, $V_m$, $P_g$, $Q_g$) and an independently auxiliary task $\lambda$.  Then, we predict task $\mu$ based on main task $X$. After that, we estimate $\mu$ based on $Z$.

%In this way, we not only include the solution variable $X$ but also predict the key factors, i.e., the Lagrange multipliers $Z, \lambda, \mu$ that impact the converge rate. In contrast, these multipliers are not considered in the existing learning-based approaches for the AC-OPF problem.


%\subsection{Network Parameters} 
%\textcolor{red}{explain why we have seven. We have four or seven? } 
%The seven estimators have different typologies, summarized in Table~\ref{tab:model_config}.  % } %The shared representative in the shadow layers takes the power load $P_d$ and $Q_d$ at each bus as inputs,  totaling 600 inputs. We use five fully-connected networks in the shared layers. The numbers of nodes for the five networks are 600, 720, 840, 960, and 1080. The five networks extract shared features and feed them to estimators. There are seven estimators, each of which is a fully-connected network customized for a task. The seven estimators have different typologies, summarized in Table~\ref{tab:model_config}.  We use ReLU as the activation function to increase the nonlinearity of our neural network.

%We discuss the four objective functions as follows.% }
%We discuss how to impose those constraints during the model construction in this section.
%While neural network models can be adjusted as a nonlinear tool box to accommodate a change of inputs and generate some approximation, the understanding of the model is lost. Instead of shifting to trust in the correctness of data mining algorithms, we seek for what variables physically mean and which physical laws are driving the interpretable evolution of the analysis paradigm.

%The solution in power grid simulation must respect several physical constraints, such as power generation constraints, line flow constraints and bus voltage constraints. 
%The neural network model must consider these physics information through exploiting the physical meaning of the power flow and the topology of power grid network. 

%Incorporating these constraints into our neural network model not only improves model accuracy but also brings benefits for quality guarantee. 

%In general, the constraints are classified into hard and soft constraints. 
% The hard constraint includes strict requirements on the value range of variables in applications; 
% The soft constraint includes domain knowledge that can be used to improve model accuracy, such as physical principles, conservation laws, and others gained from theoretical or computational studies. 
% We discuss how to impose those constraints during the model construction in this section.

%\subsection{Optimize Main tasks.}
%\label{sec6:partA}
\begin{comment}
Besides using supervised training to directly infer and score the prediction in loss function, we include external objective functions for error calibration through extracting physics information from power grid simulations. %We design data-driven approaches and properly calibrate solution with incorperating physical understanding.
We introduce four objective function incorporating domain knowledge and optimize the model parameters by minimizing the objective function. 
\end{comment}

%} \textcolor{red}{(In the above discussion, what is the connection between Equation~\ref{eq:1b} and Equation~\ref{eqn:3}?)
%The power grid simulation introduces the power flow equality constraints shown in Eqn.~\ref{eq:1b} to make the simulation of the power grid system stable and make the simulated solution feasible. We encapsulate the AC nodal power balance equations(Eqn~\ref{eqn:3}) into objective function $f_{AC}$ to guide model training, shown as follows. 
%\textcolor{red}{(explicitly tell what are inputs, outputs and physics info in the above sentence. Using one or two sentences to intuitively explain the above equation.)}

%The objective function bridges model inputs, outputs and the physics information of power networks to yield quantitatively better results.   %\textcolor{red}{("model prediction and check its feasibility" is confusing.) }}

%\textcolor{red}{(is the above description for the equation~\ref{eqn:fAC}? is there any formulation for the above description?)
%A block diagram of embedding AC physical laws in MTL training is shown in Figure~\ref{fig:ACtraining}, and shows the computational blocks related to optimize the parameters of the MTL. In power grid simulation, \textit{Domain Information:}$C_g$, $Y_{bus}$ is a fixed unit providing physical topology information.  Power loads data is input problem fed to through the MTL to produce solution $V_a, V_m, P_g, Q_g$. We integrate the AC power balance law(Eqn~\ref{eqn:fAC}) to calibrate the training in $f_{MTL}$. We first calculate the power generation based on the prediction solution$X$ and domain information$C_g$, $Y_{bus}$, and subtract power generation from power loads. We then calculate the difference between the power loads and power generation, and try to minimize the difference within the objective function $f_{AC}$.
%The data driven architecture \textcolor{red}{(what is the data-drive architecture? Consider to re-write it as follows: "The above training process is driven by xxxx data. Such a data-driven architecture xxxx" )} 
%\textcolor{red}{(what is the point you want to make in the last sentence? Why is it worth notice?)}
%The data driven architecture  mitigates the risk of obtaining infeasible solutions: the predicted solution is misleading by the noise of training date and violates the basic AC power balance law. Note that the only block with training parameters is the MTL and all blocks are differentiable.
%Embedding the objective function $f_{AC}$ has two significant benefits. First, since the information of model inputs is limited to predict its outputs, we incorporate non-trivial data-augmentation as a complementary increasing prediction accuracy. Second, we can efficiently perform transfer learning with fewer training data when the typology of power network is modified, e.g., a transmission line is suddenly broken. With this, we can improve our MTL prediction and facilitate the solution robustness. 
%\textcolor{red}{(The following paragraph and the last paragraph seem to talk about the benefit of embedding the objective function. Can we combine them together into a paragraph? )}
%by implying AC physical law.
%Incorporating the equality constraints minimizes the loss for predicting the optimization vector $X$, and also facilitate the robustness of the predicted solution by implying the physical law.
%The AC-OPF formulation includes two types of inequality constraints. The optimization vector $X$ are quantitatively bound in the \textit{explicit inequality} ($X_{min}<X<X_{max}$) and branch flow limits are included in the \textit{implicit inequality} ($H(X)>0$). For implicit inequality, we apply physics information $C_g$ and $Y_{bus}$ to to calculate the branch flow state $H(X)$ on model prediction and check its feasibility.  

%We utilize characteristics of exponential function to punish an overflow error in these inequality constraints, i.e., the prediction is out of the expected range. We first transform the explicit inequality as follows.

%\textcolor{dong}{
%We utilize exponential functions to punish the overflow error in these inequality constraints. The prediction is out of \textcolor{wq}{a limited range}, %\textcolor{red}{(a little confusing. What is the expected range? Xmin? Xmax?)}
%because of using the exponential functions. Equation~\ref{eq:ineq_constraint} shows how we use the exponential functions.%}%Where $X$ is the predicted optimization vector in MTL. Once the predicted vector $X$ violates the inequality constraints, for example, $H(X_k)<0$, the overflow error will be visibly shown up in objection function $f_{ieq}$ and gradually calibrated through backpropagation in training phrase. The main task $X$ is restricted in a quantitative way to improve simulation quality. 

%Here is a technique strategy about model training. After adding the objective function $f_{ieq}$, the training becomes unstable. There are some large updates to weights during training, causing a numerical overflow or underflow, i.e., ``exploding gradients''. We add a gradient clipping function ``clip\_grad\_norm()'' to clip gradient values that exceed a preferred range and set the default value as 5.0 in our paper.

%\textcolor{dong}{% We use the default 
%\textcolor{red}{(5.0 is the range? why 5.0?)}%}\textcolor{red}{(what is the range?)}


% Besides the above soft constraint, we add the variable bound (Eqn.~\ref{eq:1d}) on the optimization vector $X$ in our model as another soft constraint. 
% To incorporate the bound constraint into our model, we first transform the above equation as follows.
% \begin{equation}
% X-X_{min}>0,  X_{max}-X >0.
% \end{equation}
% Then, we incorporate the above inequality equations as a penalty loss in a weighted sum.
% \begin{equation} 
%     L_{ieq} = \sum_{i=1}^n w_i\times e^{( X-X_{max})}+ \sum_{i=1}^n w_i\times e^{(X_{min}-X)}
% \end{equation}
% The main task $X$ is restricted to improve prediction accuracy with an exponential penalty. 


%Note that we didn't transform the explicit inequality as hard constraints during the modeling training phase. Generally, implementing the hard constraints is normalizing the input data with variable bounds and adding a non-linear activation function(e.g., ``sigmoid'') at the last hidden layer to project predictions onto the region induced by the explicit inequality. However, normalization in the main task maps the large regions of input space to an extremely small range and weakens the feature diversity in raw data and the Sigmoid activation also causes severe gradient vanishing problem especially the input space is large.
%\textcolor{red}{(The last paragraph says "exploring the physics info", but from the above equation, I didn't see any physics info.)}

% \subsection{Optimizing auxiliary tasks}
% \label{sec6:partB}%Here, we refer classified into hard and soft constraints. 
%The hard constraint includes strict requirements on the value range of variables in applications; 
% The soft constraint includes domain knowledge that can be used to improve model accuracy, such as physical principles, conservation laws, and others gained from theoretical or computational studies.  we propose two ways constraints to incorporating , \textit{hard constraint} and \textit{soft constraint}.
% \textcolor{gokcen}{rephrase? reconstruct?}  %\textcolor{red}{(what is the connection between the last two sentences? )}%\textcolor{red}{(Should be define hard constraint and soft constraints earlier? because prior sections use the term soft and hard constraints.)}


%In the Lagrangian Eqn~\ref{eqn:largran}, Lagrangian factors $\lambda$, $\mu$ and $Z$ are embedded to satisfy such constraints.
%We construct an objective function $f_{Lag}$ to guide the training for soft constraints.%For the last part of Eqn.~\ref{eqn:largran}, $\gamma\sum_{m=1}^{n_i}\ln(Z_m) \approx  0$, we discard it because we have imposing hard constraints to ensure $Z>0$.


%Also, the Lagragian factors must respect to the strict requirements $Z>0$ and $\mu>0$. We refer the variable bounds as hard constraints.

% We impose soft constraints by modifying the loss function. 
% We choose the loss function to incorporate soft constraints because it is well known that the prediction task and sample data should guide the construction of the loss function, and the loss function has significant impacts on the solvability and generalizability of the machine learning model. 
% We impose three soft constraints in our study, power flow constraints, Lagrangian conservation, and optimizing the objective function.

%We incorporate hard constraints during the training phrase by projecting predictions onto the region induced by the constraints. Firstly, we normalize the raw data of gournd truth into a range of $[0,1]$. Then, we apply a ``sigmoid'' activation function at the last layer to bound the output range of $Z$ and $\mu$ to be positive and into the same range $[0,1]$. These techniques provides hard upper and lower bounds on prediction and guarantee its feasibility. % \textcolor{red}{(what is ``its''? 0 and 1 are the lower and upper bound? Why choose 0 and 1?)} 


%Incorporating $f_{AC}$ and $f_{ieq}$ improves the feasibility and robustness of the simulation solution $X$. $f_{f(X)}$ improves the accuracy of $X$. $f_{Lag}$ optimizes auxiliary tasks $\lambda, \mu $ and $Z$.  We compose these objective functions into loss function $L$ in Eqn~\ref{eqn:charb_loss}, and set their corresponding weights empirically. %The weights associated with the above objective functions (e.g., $w_{ieq}$ and $w_{f}$) are determined empirically. \textcolor{red}{(how do we empirically decide that? Give more comments.)}
% \begin{equation}
% \begin{split}
%   L_{total} =& w\cdot L+ w_{eqn}\cdot L_{eqn} + w_{ieq}\cdot L_{ieq} + \\
%   &w_{lag}\cdot L_{lag} + w_{f(X)}\cdot L_{f(X)} 
% \end{split}
% \end{equation}%Note that the proposed methodology of incorporating hard and soft constraints into neural network models is not only restricted in power grid simulation or optimization problems but also utilizable in other neural networks to obtain better physical understanding in many scientific applications.


% \textcolor{gokcen}{General comment for this section, is there any particular reason we follow this ordering of the physics constraints? If not, maybe it is better to follow the same order we used in the background section, equations 1a, 1b, 1c, ..Does it make sense?}\textcolor{wq}{wq: if doing so, we need to move f(x) in the beginning. I still think the AC law is better as the first one and it is a good example how we incoperate physical constraints.} %To further study the feasibility of \name, we use the outputs of \name as a warm-start point to trigger the final convergence in MIPS. 
%However, we do need to execute the model inference and we need to perform additional computation in case the generated solution is not accurate enough. To take into account these additional factors, %\textcolor{red}{should we remove the following sentence regarding the SR? We have already a section about accuracy}
%Although we achieve a $100\%$ $SR$ for 14-bus, 57-bus and 118-bus, our success rate for 30-bus and 300-bus is $97\%$ and $92\%$, respectively. %We refer Figure~\ref{fig:over_speedup}(a), which compares the execution time of numerical solver MIPS and our framework \name. %\textcolor{gokcen}{need to explain what do you mean by "the restart execution time if the simulation is not converge"? does it mean if the simulation fails, do you restart with \name or MIPS? how it is calculated?}
%We discuss \textcolor{gokcen}{performance breakdown} in greater detail in Section~\ref{sec:eva_perfmodel}, analysing framework speedup with a performance metric. \textcolor{gokcen}{what do you mean by "analysis framework speedup with a performance metric", it is confusing.}
%\textcolor{wq}{We discuss performance breakdown in greater detail in Section~\ref{sec:eva_perfmodel}, analysing the breakdown of time spent by MIPS and \name.}%The speedup relevant to execution time is considerable when solving the AC-OPF by \name versus MIPS, ranging from nearly a $2.24\times$ speedup up to over a $3.28\times$ speedup.
%\textcolor{gokcen}{can we put execution time and speedup in the same graph? it is hard to calculate the speedup from the graph?}%\textcolor{gokcen}{it is not clear what it means " execution time is continually decreased,", figure 4 does not show this, do you mean "the performance benefit of \name is more evident as the size of power networks increases, which shows a notable potential in accelerating large-scale power grid systems."}
%Note that using the results of \name as warm-start for MIPS, the solution is the same as that solved by MIPS directly.
%\textcolor{gokcen}%\textcolor{gokcen}{"iterative process" rather than "convergence process"} \textcolor{gokcen}{"computationally intensive" rather than "computation-critical"}%\textcolor{gokcen}{the number of iterations}%All input problems significantly benefit from the acceleration even including some extra overheads.  

% \textcolor{gokcen}{Is there any difference between how we calculated speedup in Figure 4, and Figure 6. I think there is no need to have a separate section for Performance breakdown. Isn't it still related to \name speedup? We can blend section 9.B into 9.A.v }\textcolor{wq}{performance breakdown is good to emphasis speedup performance and analysis where our speedup comes from.}%\textbf{Success Rate and Prediction Accuracy.} 
%The accuracy of the results produced by \name is presented in Figure~\ref{fig:err_ana}.
%\textcolor{gokcen}%\textcolor{gokcen}{ I think you don't need this sentence "Figure~\ref{fig:err_ana} shows that this is more or less true."}
%For prediction $X.Va$, $X.Vm$, $X.Pg$, $X.Qg$, $\mu$ and $z$, most of points lie above the $y=x$ line  
%\textcolor{gokcen}%For prediction $\lambda$, the predicting exists variation, in which the over-prediction and under-prediction are more or less evenly distributed. 
%\textcolor{gokcen}
%outperforms the numerical solver at most time, and can consistently provide efficient acceleration for the mission-critical applications.
% \begin{table}[!t]
% \centering
% \caption{Performance of learning based warm-start for the five problem sizes.} 
% \label{tab:model_perf}
% \begin{tabular}{l p{0.9cm}p{0.9cm}p{0.9cm}p{1.1cm}p{1.1cm}}
% \hline
% Problem size  & 14-bus & 30-bus & 57-bus & 118-bus & 300-bus \\
% \hline    
% Success rate & 100\% & 96.7\% &100\% &100\% & 80.5\%\\
% Speedup & 1.40$\times$ & 1.40$\times$ & 1.35$\times$& 1.74$\times$& 2.32$\times$ \\
% Effective ratio &$97.9\%$& $78.9\%$& $96.3\%$& $99.8\%$ &$99.7\%$ \\
% \hline
% \end{tabular}
% \end{table}

% Based on the speedup, we introduce a definition of effective ratio,
% $ER = \frac{N(SU>1)}{N_{total}}$, where $N(SU>1)$ represents the number of input problems achieves a positive speedup (more than $1\times$ speedup), and $N_{total}$ is the total number of input problems.
% We test the effective ratio to show the efficiency of acceleration on different input problems. 


% Table~\ref{tab:model_perf} shows the results of robustness, overall speedup, and effective ratio.
% Table~\ref{tab:model_perf} reveals that \name provides a relatively high success rate in all test systems. 

%\textcolor{review}{Review4:The success rate gets dropped in some cases and speedup is not attractive. (2) The samples of neural networks need to be more diversified to show the feasibility for real situations.}

% We further test the effective ratio of \name.
% The results in Table~\ref{tab:model_perf} shows \name outperforms the numerical solver at most time, and can consistently provide efficient acceleration for the mission-critical applications.
% Note that using the results of \name as warm-start for MIPS, the solution is the same as that solved by MIPS directly.
%\textcolor{review}{Review1: Why does the model for 300-bus have the highest speedup but the lowest success rate? And the model for 57-bus has low speedup but always success.}

%\subsection{Performance Breakdown}
%\label{sec:eva_perfmodel}
%\begin{figure}[!t]
%  \centering
%  \includegraphics[width=1.0\linewidth]{Figures/perf_breakdown.pdf}
%      \vspace{-20pt}
%  \caption{Execution time breakdown}
%  \label{fig:per_bd} 
%  \vspace{-20pt}
%\end{figure}


%We introduce a performance metric to evaluate the speedup:
%\begin{equation}
%  \label{eqn:speedup}
%  SU = \frac{T_{MIPS}}{T_{MTL}+T'_{MIPS} +T_{MIPS}\times(1-SR)}  
%\end{equation} 
%where $T_{MIPS}$ represents the solving time with MIPS, $T_{MTL}$ represents the execution time of MTL, and $T'_{MIPS}$ represents the convergence time in MIPS initializing with the output of \name. $T_{MIPS}\times(1-SR)$ calculates the restart execution time with MIPS if the simulation fails.
%%\textcolor{gokcen}{I am not sure if I understood this formula. what is "n"?  what is the difference between $T^{MIPS'}$ and $T^{MIPS'}{i}$?}
%We use SR to represent the overall success rate, $SR = N_{suc}/N_{total}$, where $N_{suc}$ represents the number of problems successfully solved and $N_{total}$ represents the total number of input problems.
%%\textcolor{gokcen}{the formula SR is not correct on the pdf. please have a look at it.}
%In particular, we achieve a $100\%$ $SR$ for 14-bus, 57-bus and 118-bus while providing $97\%$ and $92\%$ $SR$ for 30-bus and 300-bus respectively. 
%%\textcolor{gokcen}{the SR is hidden in the text, we have very good success rate. we have to make sure that it is obvious. we should highlight it when we talk about speedup.
%%If you would like to have another section like speedup, convergence, etc. Feasibility of the solution (SR) should come soon after speedup. if we need space, we can merge speedup and convergence into the same section, after all speedup and iterations numbers are more or less the same.}
%If the "warm-start" solution from the neural networks does not lead to a proper solution by the numerical solver, we will restart these failure cases from scratch. 
%We include the restart overhead in the overall speedup. Hence, we guarantee a 100\% success rate in practice.

%Neural Network (NN), as a tool to learn and model complicated (non)linear relationships between input and output data sets, has shown preliminary success in some HPC problems (e.g., detecting neutrinos~\cite{ichep16:radovic}, climate simulations~\cite{nips17:racha}, and fluid dynamic simulation~\cite{dong2019adaptive}). 
%With neural networks, scientists are able to augment existing scientific simulations by improving simulation accuracy and significantly reducing latency~\cite{richard2014artificial, sr15:widley, mathuriya2018cosmoflow, balaprakash2019scalable, yang2019highly,liu2019tomogan,liu2019deep}. %Neural networks have been applied to solve the optimal power flow  problem~\cite{guha2019machine, baker2019learning, zamzam2019learning}. However, those existing efforts have a fundamental limitation. They use neural networks to approximate the whole simulation and generate an approximate solution or facilitate existing solvers by identifying the active constraints~\cite{deka2019learning, ng2018statistical}. Because the neural network provides only an \textit{approximation} of the optimal solution or approximates computation in the simulation, these efforts cannot provide the optimality of the solution. 
%\textcolor{gokcen}{which is guaranteed by the numerical solver run at the back end of the process.}
%\textcolor{gokcen}{However, there is a lack of systematic approach to quantify sensitivity.}
%and includes a sensitivity study tool. The tool isolates %and using neural network prediction for other variables. %by using ground truth for some variables and using neural network prediction for other variables. %The sensitivity study for execution time guides on the model topology design.%building loss function for improving model robustness; %power grid simulation;

%\item Using 10,000 problems as the simulation input for evaluation and using the original AC-OPF simulation as a baseline, \name achieves $2.60\times$ speedup on average (with the consideration of NN cost), up to $3.28\times$, without losing the optimality of the final solution.
%To further explore the performance improvement by \name, %Figure~\ref{fig:per_bd} shows the runtime breakdown of MIPS and \name, normalized to the overall runtime where the problems run with MIPS.
%The pre-processing refers the execution time of problem construction and data preparing in MIPS, in which MIPS and \name show almost the same processing time.
%The Newton update represent the execution time spent in Newton iteration.
%\name have extra overhead about the execution time of MLT for generating warm-start solution and the restart time with failure cases.
%As Figure~\ref{fig:per_bd} depicts, \name is effective at reducing the time spent on the convergence, i.e., Newton Update. 
%\name demonstrates significant performance improvement for input problems despite the extra overhead introduced by the MTL model.
%%All input problems significantly benefit from the acceleration even including some extra overheads.  

%% \textcolor{gokcen}{Is there any difference between how we calculated speedup in Figure 4, and Figure 6. I think there is no need to have a separate section for Performance breakdown. Isn't it still related to \name speedup? We can blend section 9.B into 9.A.v }\textcolor{wq}{performance breakdown is good to emphasis speedup performance and analysis where our speedup comes from.}%\textcolor{gokcen}{say it first why we compare with separated neural networks}
%we set up the model with multiple separated neural networks to show the efficiency of multitask learning, in which each neural network is used to predict a specific task individually.%In this section we use ``MTL'' to represent the multitask learning model without incorporating physical constraints ans use ``\name'' to represent the multitask learning model with physical constraints.%MTL offers $36\%$ average speedup and $22.5\%$ average success rate improvement compared to the multiple separated models. %\textcolor{gokcen}{do you have any idea why the multiple separated neural networks presents poor speedup? do you know what it is missing?}%As the previous Section shows, using separate NNs greatly reduces the accuracy of the solution.
%The prediction accuracy of neural networks can not be precisely bound due to the uncertainty of neural networks.
%To fairly compare with the %We first directly use \name to replace the entire solving process in MIPS and test the performance of . 
%when the output of \name is used as a warm-start point to solve the AC-OPF problem.
%\textcolor{gk}{I am a little confused here a little, in this sub-section, we replace the entire computation with the NN model, so why do we start the sentence with "warm-start"?}
%We take the MIPS solver as the baseline method. MIPS is the traditional method used in the Matpower and does not include any neural network.
%Compared with neural network-based acceleration, MIPS has the highest simulation quality, but the performance is limited. All performance (execution time) reported in this section is shown as ``speedup'' concerning the performance of MIPS.
%\textcolor{review}{Review4:Directly using the predicted solutions of neural networks will cause a wrong solution and may not be accepted as a physical solution.}
%We involve two factors here to measure the performance.

%\textcolor{dong}{\textcolor{red}{(in the above discussion, we are using ``soft constraints''? what is ``hard constraints''?)}
%\textcolor{gokcen}{add a sentence to summarize the benefit of adding "Guarding Inequality Constraints" into our model, as conclusion}


% However, there are three main drawbacks by doing so.
% \textit{First}, in the ground truth data set, the values of most variables in $X$ gather into a small range, rather than widely spread into the range bounded by the boundaries $X_{min}$ and $X_{max}$. This means that if we normalize $X$ by the boundaries, we expand the prediction range and can significantly decrease the prediction accuracy. 
% \textit{Second}, after normalization, the difference of variable ranges is weakened. 
% Normalization rescales the original range of variable values into the range of [0,1] through simple transformation. However, the values of most variables have a rather large range. For example, the value range of $P_g$ is [0,2030]. Mapping the large range to the small range of [0,1], we decrease the sample diversity and have the risk of losing some invisible information. 
% \textit{Third}, if we use normalization, experiments show that many inputs are mapped to very similar outputs. 
% This is due to a severe gradient vanishing problem in our model after using the sigmoid activation function. 
% The sigmoid activation maps the large regions of input space to an extremely small range. In these regions of the input space, a large perturbation of the input only brings about a small variance on the output. This becomes even worse when we stack multiple neural network layers on top of each other.

% To apply the above soft constraints, we can use the normalization and ``sigmoid'' activation to bound the range of $X$. 

%In particular, the formulation of the AC-OPF problem in Eqn.~\ref{eqn:largran} imposes a constraint on the Lagrangian multiplier $Z$, i.e., $Z>0$. 


% We incorporate the implicit inequality as soft constraints and explicit inequality as hard constraints.
% The hard constraints are strict requirements on the value range of variables in applications. We incorporate hard constraints during the training phrase by projecting predictions onto the region induced by the constraints.

% The soft constraint includes domain knowledge that can be used to improve model accuracy, such as physical principles, conservation laws, and others gained from theoretical or computational studies. %The optimization goal of the AC-OPF is to minimize the objective function $f(X)$. We explore the physics information of how to construct the cost function and minimize the loss between the predicted cost and ground truth cost.
% In general, $L_1$ loss is a common method to calculate output loss in neural network models.
% \begin{equation}
%     L1  =  \frac{1}{|\mathcal{V}|}\sum_{v\in \mathcal{V}} |v - v_{gt}|,
%     \label{eqn:l1_loss}
% \end{equation}
% where $v$ is model output and $v_{gt}$ is the corresponding ground truth.%We use a variant of $L_1$ loss~\cite{janocha2017loss}, the Charbonnier loss, as our loss function. The supervised loss function calculates the difference between each of the predicted output variables $v$ and the corresponding ground-truth value $v_{gt}$ collected by running the MIPS solver. Our loss function is defined as follows. 

%where the set $\mathcal{V}$ comprises of $V_a$, $V_m$, $P_g$, $Q_g$, $Z$, $\lambda$ and $\mu$, $W_v $ is the corresponding weight on each task and $\epsilon$ is a small constant for numerical stability. We set $\epsilon$ as $1e-9$ in our study.
% \textbf{Pre-processing.} %and Post-processing}
% \label{sec5-3}

%The ranges of features $X, Z,\lambda,\mu$ are quite different from each other. For example, consider two features in bus-30. The power generation on the 2nd bus ranges from [21.70, 23.86], while a value in $Z$ ranges from [3.11e-11, 1.92e-07].
%\textcolor{red}{(is this range for $X$?)}%\textcolor{red}{(Add one or two sentences to explain why the value difference is a problem)}%\textcolor{gokcen}{can we add references here for these techniques?}
%\textcolor{red}{(the following discussion o normalization and standarization can be simplified, if we don't have enough space. )}
% 1)Normalization.
%Just as modeling systems require the development and analysis of specialized structure-exploiting methods for optimization, realizing the benefits of scientific machine learning will require similar recognition of problem structure in scientific applications. In this section, we develop a tool to perform sensitivity study for modeling design. We explore feature sensitivities around a solution, and quantities the impacts to simulation quality, which inversely used for feature selection and prioritization.


% We first initialize different parameters as inputs to simulation convergence.
% %We then develop a quality-prior model design mechanism, which significantly mitigated the training overhead of inefficient model evolution. 
% We conduct extensive experiments to study the effect of different input components to the success rate and acceleration of simulation.
% In scientific applications, variables have different importance and contain complex relationships among data set.
% And especially when the variables in scientific applications are initialized by low-precise prediction of neural networks, it could decrease the success rate of simulation and even causes a crash.
%\textcolor{wq}{Sensitivity study leverages \textit{component analysis} to determines features critical to the simulation convergence for model outputs and \textit{quantity analysis} evaluates the impact of the noisy features for model topology design. }
%\textcolor{gokcen}{(I will move the following sentence as a last sentence of this parag.. Because the next sentence moves back to how we have selected these variables.)}

%\name choose variables critical to the simulation convergence as features. %First, we perform component analysis for feature selection. We check the convergence criteria in MIPS source code, which shows features $X, \lambda$, $\mu$, $Z$ jointly contribute to the simulation convergence.  Hence, our model involves multi-objective prediction and we take features $X, \lambda$, $\mu$, $Z$ as outputs of our neural network model.
%\textcolor{wq}{(delete?}{Based on the problem formulation in Section~\ref{sec:acopf}, we first include the optimization variable $X$ in Eqn.~\ref{eq:xvariable} as a candidate feature.
%Also, we involve Lagrangian factors $\lambda$, $\mu$, $Z$ in Eqn.~\ref{eqn:largran} as these features are important factors involved in the solving process of Lagrangian formulation. }\textcolor{wq}{delete?)}
%\textcolor{red}{(re-write the following paragraph. Put the discussion in the context of our problem. For example, you can say that using the four variables as the output of the prediction model, we need some guidance on the model topology and xxxx, and a good model topology and xxxx are important to improve modeling accuracy.) }
%A neural network model intuitively build without such knowledge will becomes a opaque black box and hard to fully exploit the model benefits. The inaccurate prediction used for scientific simulation may decrease the simulation quality and even case a crash. We perform a quantity analysis to understand the effects of prediction accuracy to simulation, which is used for features prioritization and topology design of neural network model}
%While, in scientific applications, features have different importance and contain complex relationships among dataset. Intuitively building a neural network model to project these features becomes a opaque black box hard to fully exploit the potential of prediction accuracy. Once injecting inaccurate neural networks prediction, the introduced uncertainty may decrease success rate of simulation convergence and even causes a crash.  We perform a quantity analysis to understand the interacting effects of features, which is used for features prioritization and topology design of neural network model.  
%\textcolor{gokcen}%of neural network prediction, what the max speedup can be achieved if the neural network predicts all the parameters preciously. %\textcolor{red}{(I get lost here... Why do we need to ``mimic'' the lower and upper bound? What is the connection between the last paragraph and this paragraph?)}

%\textcolor{gokcen}{(I think you want to say "determine" rather than "mimic", what the max speedup can be achieved if the neural network predicts all the parameters preciously, is that correct?)}%\textcolor{gokcen}{(i think it is not obvious from the text that default data is the initial value before the simulation starts, precise data is the final value after the simulation converges. We might need to find a better, descriptive name for these two types of data.)}

%\textcolor{red}{(I got lost here. Why do we need to do the above?)}%\textcolor{gokcen}{(I usually use the same term for critical metrics.
%For examples, success rate and simulation execution time, in the last there paragraph, there are three different terms, "simulation  quality  and  execution  time", "simulation robustness  and  acceleration", and "success rate". I am not saying that we should always use the same wording but maybe better not to introduce many new terms. Just a suggestion.)}
%\textcolor{red}{(How to "inject"  the data into source code? Give a little details here. )}
%The simulation robustness refers to the success rate of final convergence, while the acceleration relates to speedup that achieved due a good initialization.  
% \textcolor{wq}{
% Simulation robustness should be aware of the \textit{success rate} of final convergence, namely the ratio of those initial solution with which the power gird simulation can reach the convergence criteria to the total number of input problems.
% \textcolor{gokcen}{(what do you mean by "should be aware of?", do you mean "represents or refers"?)}
% Simulation acceleration refers to the \textit{speedup} about execution time, namely the rate of change using different initial points in power grid simulation.
% \textcolor{gokcen}{(I think we need a simpler description about the speedup, I feel like it is a little confusing)}        %\textcolor{gokcen}{ a quicker convergence  -- > high speedup}%\textcolor{red}{(define ``success rate'' and ``speedup'' somewhere. )} 
%Hence, we generate as many as $2^4$ combinations of rough and precise data in four features and record their related success rates and speedups of different cases. 
%\textcolor{dong}{
%As shown in Table~\ref{tab:Ablation}, we include $16$ cases to initialize the solving process and test the success rate and speedup.  In each case, we use marker ``0'' to represent rough data and use ``1'' to represent precise data. We set the baseline that all variables ($X$, $\lambda$, $\mu$ and $Z$) are initialized with rough data and use the baseline to measure the success rate and speedups of the other 15 cases on eight test systems. From Table~\ref{tab:Ablation}, we have the following observations: %\item \textbf{Observation 1}: Optimization vector $X$ and Lagrangian factor $\lambda$, $\mu$ and $Z$ are interacting. Features $X$, $\lambda$, $\mu$ and $Z$ jointly contribute to a quick and success convergence (case \uppercase\expandafter{\romannumeral 16}); Initializing without the precise optimization vector $X$(case \uppercase\expandafter{\romannumeral2}-\uppercase\expandafter{\romannumeral8}) easily cause a crash; Only starting with precise $X$(case \uppercase\expandafter{\romannumeral9}) maintains $100\%$ success rate but leave the performance opportunities on the table.

    %ation 1}: Precise $X$ maintains a $100\%$ success rate(case \uppercase\expandafter{\romannumeral9}), while features $X$, $\lambda$, $\mu$ and $Z$ jointly contribute to a quick and success convergence (case \uppercase\expandafter{\romannumeral 16}). 
    %\item \textbf{Observation 2}: For success rate and speedup, feature $\lambda$ is relatively independent, and $Z$ has a strong reliance on $\mu$. For feature $lambda$, starting with only a precise $\lambda$, the solving process can achieve a $100\%$ success rate(cases \uppercase\expandafter{\romannumeral5}, \uppercase\expandafter{\romannumeral13}) while involving other Lagrangian factors ($\mu$ or $Z$), success rate decreased(\uppercase\expandafter{\romannumeral6}, \uppercase\expandafter{\romannumeral7}, \uppercase\expandafter{\romannumeral14} and \uppercase\expandafter{\romannumeral15}). For features $Z$ and $\mu$, only initialized with precise $Z$, the success rate is pretty low(cases \uppercase\expandafter{\romannumeral2}, \uppercase\expandafter{\romannumeral10}) but initialized with both precise $Z$ and $\mu$, the solving process is still stable(cases \uppercase\expandafter{\romannumeral4}, \uppercase\expandafter{\romannumeral8}, \uppercase\expandafter{\romannumeral12}, and \uppercase\expandafter{\romannumeral16}).   %\textcolor{red}{finish the above sentence.}%\textcolor{red}{finish the above sentence.}
    

    %\item \textbf{Observation 3}: Features $X$, $\lambda$, $\mu$ and $Z$ have dependency and the over performance of success rate and speedup can not be accumulated by accuracy improvement of a certain feature(comparing case \uppercase\expandafter{\romannumeral9} with \uppercase\expandafter{\romannumeral10}). 
    
    %\textcolor{red}{(re-writing the following paragraph. It's confusing.)}%\item \textbf{Observation 4}:  $X$, $\lambda$, $\mu$ and $Z$ have dependency and the over performance of success rate and speedup can not be accumulated by accuracy improvement of a certain feature(comparing case \uppercase\expandafter{\romannumeral9} with \uppercase\expandafter{\romannumeral10}). 
    
    
    % \item\textbf{Observation 3}: $Z$ has a strong reliance on $\mu$. In Lagrangian factors, if we only initialize the solver with precise value of $Z$, the success rate is pretty low, which is observed from cases \uppercase\expandafter{\romannumeral2} and \uppercase\expandafter{\romannumeral10}; Also, if we initialize with a precise $Z$ and $\mu$, the solving process is still stable, observing from cases \uppercase\expandafter{\romannumeral4}, \uppercase\expandafter{\romannumeral8}, \uppercase\expandafter{\romannumeral12}, and \uppercase\expandafter{\romannumeral16}.
%\textcolor{red}{(what is ``multi-objective''?)}\textcolor{red}{between the object 1 and ``feature priority'', there is a missing link. Can you make the link here? For example, you can say that "since A has dependency on B, we should make B very accurate. Hence we give B high priority". What is "priority"? It is not clear.}
%\textcolor{red}{(define the term "dependency between features ", so that you can use it in the rest of the paper)}

%\textcolor{red}{(re-write the following sentence. confusing. )}
%In observations 2 and 4, features show domain specific characteristics which may relevant to physical knowledge in power grid simulation.   \textcolor{red}{(It's not clear to me how the observations 2 and 4 can lead to the above conclusion...)}
%In observation 3, features shows different characteristics relevant to  
%In Eqn.~\ref{eqn:largran}, we can also observe multiplier $\lambda$ is related to the equality constraints $G(X)$ while multiplier $\mu$ and $Z$ are associated with the inequality constraints $H(X)$. 

%\textcolor{gokcen}{it is also not clear to me how observation 2 and 4 are connected with the domain specific characteristics. I thought we looked at the initial formulation of the problem to identify some of these dependencies.}

% From these observations, components $X, Z, \lambda$, and $\mu$ have inner connections, which should be considered in our neural network model construction. Only starting with $\lambda$ and one of another multiplier ($\mu$ or $Z$), the inequality constraint $\mathbf{\mu}^\intercal(H(X)+Z)=0$ can not be satisfied, and initializing with inequality multiplier $\mu$ or $Z$ can not fulfill the equality constraint.

% so the importance of variables can be expressed as:
%  \begin{equation}
% \label{eqn:7}
%     W_{X,Z,(\lambda,\mu)} = \sum\limits^{\vbox to 0pt{\hbox{\rule{.5pt}{1ex}}}}_{ k \in obser} \one\{X=1,Z=1,(\lambda=\mu)\} \cdot \{SR_{k}\} ,
% \end{equation}
% where $W_{X,Z,(\lambda,\mu)}$ represents weights of the four variables by averaging the success rate ($SR$)) of these cases that satisfy corresponding observation, and $\lambda$ and $\mu$ share the same weight. $SR_{k}$ and $SU_{k}$ are obtained from Table \ref{tab:Ablation}. Then these weights represent the importance of related variables and are used to construct the loss function (Eqn.~\ref{eqn:l1_loss}).%Based on observations in Section~\ref{sec:sensi_study},.
%The interactive learning model is implemented to share information between these tasks. 
%Compared to using multiple separate models for each task, using the multi-task learning model we can share information from the shared layers in the model while customizing specific layers for corresponding tasks. 
%The shared layers capture information common to tasks, while the task-specific layers capture information specific to each task.
%\textcolor{red}{(what is auxiliary task?)}\textcolor{red}{(what is the main task?)}%The generalization performance of the main task can be improved by leveraging the domain-specific information from the auxiliary tasks.

%\textbf{Info-interacting in shared layers.} %Observations 1 and 3 reveal that feature $X, \lambda, \mu, Z$ are correlated, and each of the three features is sensitive to %precise variation of other three features
%accuracy of other three features.%\textcolor{gokcen}{why only observation 1 and 3 reveal that these four features are correlated? what about other 2? Also, it is not clear to me what "each of the three features" refers to? I believe here we simply would like to say there is correlation among these four features and we would like to leverage this relations in our model, is that correct?}
%We utilize parameter sharing and loss sharing to enable information interaction.%\textcolor{dong}{(How does the first sentence of this paragraph related to the second sentence of this paragraph?)}
%\textcolor{red}{(re-write the above sentence. Who have inner connections? What are ``inner connections''? )}
%Besides the shared representation in shared layers, the multitask learning model has task-specific layers to specialize in each task. 
%We exploit task-specific layers to customize modeling design for each task.
%\textcolor{gokcen}{I would recommend using the same terms in the text and the title for "shared layers" and "task-specific layer". currently it looks like "shared layers" and "deeper layers" from the title.}
%Figure~\ref{fig:MTL} shows our design. % \textcolor{red}{(Why do we add the above discussion here? The above discussion shows the general MTL topology. Maybe it should be placed at the end of this section or at the beginning of Section VI.A.)}
% \textcolor{gokcen}{I also think that it might be better to put this parag. at the end of the previous section}
%\textcolor{gokcen}%\subsection{Tailored Design}%Although multitask learning has been showcased to achieve high prediction accuracy in various fields~\cite{zhang2014facial,xue2007multi}, multitask learning faces a range of challenges on feature selection~\cite{argyriou2007multi, obozinski2006multi}, such as reducing data complexity in high-dimensional and noisy input data with uncertainty and keeping the validity of efficient tasks.


%We show our design of MTL in Figure~\ref{fig:MTL}. Given a power network topology, we use the power load(including both the active part $P_d$ and reactive part $Q_d$) as the input and approximate multiple tasks $X, \lambda, \mu, Z$. In the MTL, the shared layers are extracting common features for different tasks in shallow layers, while the task-specific layers(estimators) borrow the information from those common features to generate their own dedicated results. Besides exploiting benefits from traditional shared layers and task-specific layers, we develop tailored design, i.e., feature prioritization and a physics-dependent hierarchy, based on quality analysis.




%Besides exploiting benefits from traditional shared layers and task-specific layers, we introduce a domain-specific design (i.e., feature prioritization and a physics-dependent hierarchy}.%\textcolor{gokcen}{let's decide "a physics-dependent hierarchy" or "enforcing prediction order", I would for the first one.}


%The outputs of the main task and auxiliary tasks are used as an initial solution to accelerate the solving process of the original power grid simulation.%The shared layers first take in load injection $P_d$ and $Q_d$ in Eqn.~\ref{eqn:3} as inputs. The shared layers are responsible for extracting common features for different tasks, while the task-specific layers borrow the information from those common features to generate their own dedicated results. Given the power load as input, the learning model is then applied to predict seven variables, including four main tasks ($V_a$, $V_m$, $P_g$, $Q_g$) and three auxiliary tasks ($\lambda$, $\mu$, $Z$).
%\textcolor{gokcen}{$\mu$ in Figure 2, looks like "u"}%\textcolor{gokcen}{here is the first time, we call it "auxiliary task".} \textcolor{red}{This is implemented by xxxxxxxxx.}
%By doing so, prediction of $\lambda$, $\mu$ and $Z$ are used as an augmentation to provide additional information for the main task. 
%In auxiliary tasks, we apply ``detach()" method to disables automatic differentiation, i.e stops keeping track of gradients in model training. We aim to learn the direct solution $X$ in the main task to guarantee simulation quantity while estimating the Lagrangian factors $\lambda$, $\mu$, and $Z$ in the auxiliary tasks to maximize the speedup performance.

%Figure~\ref{fig:overview} shows the workflow of \name, which is divided into offline and online phases. During the offline phase, we take the numerical solver (MIPS) to generates training data in power grid simulation. We inject various input problems (power loads) into MIPS and collect potential features about solutions.  
%\textcolor{red}{(sensitivity study actually does not ``select'' anything. Should we use the word ``select''?)}
%A set of high-dimensional variables in MIPS form a search space to decide which ones should be selected as features. Sensitivity study explores the space to choose features. %determine an optimal design, both of model topology and feature selection, according to success and performance (speedup) metrics. 
%\textcolor{dong}{Sensitivity study chooses those variables critical to the simulation convergence as candidates, and then uses component analysis to quantify the impact of the noisy variables (i.e., the variables with some accuracy loss) on simulation success and performance (execution time). The component analysis prioritize those variables for \textcolor{red}{xxxxxxx}. Component  analysis also studies the interacting effects of variables and the impact of the effects on simulation success and performance.  }
%Component analysis in sensitivity study is used to explore parameter sensitivities for success rate and filter features for neural network model thought triggering source code with precise or noise inputs. Meanwhile, \name analyzes interactions between inputs based on the quantity results(speedup) and decides the feature prioritization combining physical domain knowledge.

%First, \name introduces a tool, \textit{sensitivity study}, to analyze potential features and guide neural network model design. Sensitivity study (Section~\ref{sec:sensi_study}) seeks to explore the high-dimensional feature space to determine an optimal design, both of model topology and feature selection, according to success and performance(speedup) metrics. Component analysis in sensitivity study is used to explore parameter sensitivities for success rate and filter features for neural network model thought triggering source code with precise or noise inputs. Meanwhile, \name analyzes interactions between inputs based on the quantity results(speedup) and decides the feature prioritization combining physical domain knowledge.


%Next, \name designs the topology of the neural network model based on the selected features. Since multiple objects are involved in the solving process of the AC-OPF problems, we perform a multitask learning model(Section~\ref{sec:multitask}) to share domain information while customizing a specific design for each predicted task. Feature prioritization is also implied in the topology design with a physics-dependent hierarchy.%\textcolor{red}{(If you use ``MTL'' to stand for multi-task learning model here, then use MTL instead of "multi-task learning model" in the rest of the paper. If ``MTL'' stands for multi-task learning model, don't use the word ``MTL model'' for ``MTL'' in the rest of the paper)}. 
%\textcolor{dong}{
%Next, \name constructs the multi-task learning model based on the selected features (Section~\ref{sec:multitask}). The model shares domain information between prediction tasks, while uses a customized design for each task. Feature prioritization is also implied in the topology design of the model} \textcolor{red}{by a physics-dependent hierarchy.}

%Moreover, \name incorporates physical domain knowledge in model training for quantitatively better predictions (Section~\ref{sec:physics_info}). Physical constraints provide explicit and implicit error bounds which are imposed in model prediction to improve accuracy. Physical laws integrate domain knowledge to calibrate errors. The integration improves accuracy, interpretability, and defensibility of multitask learning (MTL) models while simultaneously augmenting non-trivial data as complementary and accelerating MTL model training.


% and to apportion uncertainty in a quantity of interest among uncertain inputs and their interactions (global sensitivity analysis), which in turn can be used for factor prioritization and factor
% fixing
%To systematically design a model structure, we introduce a tool to perform a sensitivity study (Section~\ref{sec:sensi_study}) as the bedrock of modeling design. 
%In sensitivity study, we perform feature selection and prioritization.
%During the model construction, we build the topology of neural network model based on observations from sensitivity study.
%In the sensitivity study, we include component analysis and prior analysis. 
%The component analysis is a quality-oriented design for success rate. 
%We analyze the importance of each variable concerning simulation success rate and qualities the importance of weights imposed into loss function. 
%The prior analysis is a light-weighted mechanism to guide model evolution. In each evolution, the prior analysis adopts a perturbed ground truth to probe the most efficient evolution direction. 

%After the sensitivity study, we build a multitask model and train it with given training data (Section~\ref{sec:multitask}). \name further extracts physical information of the simulated power network as data complementary and error calibration (Section~\ref{sec:physics_info}). %\textcolor{red}{what is the op vector?}%generator injections (\textcolor{red}{(the generator injection is $X$?)}). %Equality constraints $G(X)$ are the power balance equations incorporating variable bounds. Inequality constraints $H(X)$ are the branch flow limits. The optimization vector bounds $X_{min}$ and $X_{max}$ include the limitations of reference bus angles, voltage magnitudes and generator injections.
%\textcolor{red}{(re-write the following paragraph. It's confusing)}
%The optimization vector $X$ for the standard AC-OPF problem consists of $n_b \times 1$ vectors of voltage angles $V_a$, $n_b \times 1$ ($n_b$: number of buses) vectors of voltage magnitudes $V_m$, $n_g \times 1$ ($n_g$: number of generator) vectors of generator real power injections $P_g$ and $n_g \times 1$ vectors of reactive power injections $Q_g$.
%\textcolor{red}{(re-write the following paragraph.)}
%In the traditional formulation of the AC power flow problem, the power balance formulation in Eqn~\ref{eq:1b} is split into its real and reactive components. For a power grid network, the nodal bus injections ($P_i$ and $Q_i$) are matched to the power loads ($P_d$ and $Q_d$) and the impedance consumption($P_{bus}$ and $Q_{bus}$), which forms the AC nodal power balance equations.%\textcolor{red}{(the following sentence is confusing. which power balance equation?)}  The power balance equation ensures that the power and voltage keep constant, and represents the AC-steady conditions of the power grid system.%Matpower applies its own solver, called MIPS (Matlab Interior Point Solver). 
%}%of positive slack variables $Z$, $H(X)+Z=0$, %and using a barrier function $\ln(Z)$ to bound the slack variables. The Lagrangian formulation for the AC-OPF problem is built as follows.
%in the AC-OPF problem. 
% When the partial derivatives of Eqn~\ref{eqn:largran} are set to zero, the first order optimality conditions for the AC-OPF problem are satisfied. \textcolor{red}{(what is the "first order optimality conditions"?)}
% %}
%  \begin{equation}
%  \label{eq:5}
%   \begin{split} F(X,&Z,\lambda,\mu)=0\\
%      &Z>0\\
%      &\mu>0,
%      \end{split}
%  \end{equation}
% where $F_x$ donates the first derivatives, e.g., $F_x = \frac{\partial F}{\partial x}.$  \textcolor{red}{(what is equation 5? They are the partial derivatives of Equation 4?)}%which involves large computation overhead that iteratively converges to meet convergence criteria (four terminate conditions). In each iteration of the Newton method, the Newton update can be written as follows:


%  \begin{gather}
%  \label{eq:BBD}
%   \begin{bmatrix}
%   F_X &  F_Z &  F_\lambda &  F_\mu
%   \end{bmatrix}
%   \begin{bmatrix}
%      \Delta X \\ \Delta Z \\ \Delta \lambda  \\ \Delta \mu 
%   \end{bmatrix}
%   = -F(X,Z,\lambda,\mu).
%  \end{gather}

% In each iteration of the Newton method, the computation follows the order of (1) computing $\Delta X$ and $\Delta \lambda$; (2) computing $\Delta Z$ based on $\Delta X$; and (3) computing $\Delta \mu$ based on $\Delta X$ and $\Delta Z$. 

%In each Newton step, the computation follows the order of (1) computing $\Delta X$ and $\Delta \lambda$; (2) computing $\Delta Z$ based on $\Delta X$; and (3) computing $\Delta \mu$ based on $\Delta X$ and $\Delta Z$. 
%With MIPS solvers, a large number of iterations must be performed to produce an adequately small residual and MIPS check the feasibility of solution with four terminate conditions.

% \begin{algorithm}%[!t] 
% \caption{Primal-Dual Interior Point Algorithm}
% \label{alg:FilterLine-search}
% \begin{algorithmic}[1]
% %\REQUIRE Feastol; Gradtol; Comptol; Objectol;
% \STATE \textbf{Initialization. }start point $x_0$; Lagrangian factors $\lambda_0$, $\mu_0$, $Z_0$; perturbation parameter $\gamma$.
% \STATE \textbf{do}
% \bdwqindent
% \STATE  Calculate first derivatives of each variable ($F_X$, $F_Z$,  $F_\lambda$, $F_\mu$) based on Eqn~\ref{eq:5};

% \STATE \textbf{Newton Update Step:} 
%  \bwqindent
% \STATE Calculate the first order optimality conditions:  \begin{gather}
%  \label{eq:BBD}
%   \begin{bmatrix}
%   F_X &  F_Z &  F_\lambda &  F_\mu
%   \end{bmatrix}
%   \begin{bmatrix}
%      \Delta X \\ \Delta Z \\ \Delta \lambda  \\ \Delta \mu 
%   \end{bmatrix}
%   = -F(X,Z,\lambda,\mu)
%     \end{gather}
% \STATE Calculate $\Delta X$ and $\Delta \lambda$;
% \STATE Calculate $\Delta \mu$ based on $\Delta X$ and $\Delta Z$; 
% \STATE Calculate $\Delta Z$ based on $\Delta X$ and $\gamma$;
% \ewqindent

% \STATE \textbf{Update solution:} 
%  \bwqindent
%     \STATE update the solution $X \leftarrow X+\Delta X$;
%     \STATE update Largragian factors $Z \leftarrow Z+\Delta Z$; $\lambda\leftarrow\lambda+\Delta \lambda$; $\mu\leftarrow\mu+\Delta\mu$;
%     \STATE update perturbation parameter $\gamma \leftarrow Z^{T}\mu$;
% \ewqindent

% % \STATE \textbf{Convergence check:} 
% %  \bwqindent
% %     \STATE check feasibility condition(FC);
% %     \STATE check gradient condition(GC); 
% %     \STATE check complementarity condition(CC);
% %     \STATE check objective condition(OC); 
% % \ewqindent
% \edwqindent
% \STATE \textbf{While} $X, Z, \lambda, \mu$ satisfy terminate conditions
% \RETURN 
% \end{algorithmic}
% \end{algorithm}


%The success rate $SR$ represents the success ratio of final convergence initializing with MTL prediction.  %All restart cases are counted as failure cases. Even though the result shows the success rate dropped, we guarantee a 100\% success rate in practice.
% In this section, we study the impact of imposing physics constraints. 
% We compare the \textit{overall speedup} of our model \name with and without physics constraints. 
% Similar to Section~\ref{sec:8-2}, we use the speedup in Eqn.~\ref{eqn:speedup} to test the efficiency of physics constraints.%The proportion of positive speedup are $97.9\%$, $78.9\%$, $96.3\%$, $99.8\%$ and $99.7\%$ on bus-14, bus-30, bus-57, bus-118, bus-300 input problem respectively, which means it outperforms the numeral solver in real applications at most time.  
%\textcolor{gk}{I am not sure about the results above, do you mean 1.97, 1.78, etc.? }
% \begin{figure}[!t]
%   \centering
%   \includegraphics[width=0.8\linewidth]{Figures/sec7_loss.pdf}
%   \caption{Training loss of different models}
%   \label{fig:sec7_loss} 
% \end{figure}
% To further study the model performance of \name, we analyze the model training loss with various test systems. 
% Figure~\ref{fig:sec7_loss} presents the training loss curves of the above five test systems.
% The solid lines represent \name with physics constraints, and the dashed lines represent \name without physics constraints.
% We find that the convergence speed of \name with physics constraints is faster than those without physics constraints and achieves higher prediction accuracy and lower training loss. 
% Note that we do not introduce any extra overhead with imposing physics constraints during model prediction. We involve the physics constraints in the loss function, which is only used to guide the model training and conducted offline.

%The solving process of the AC-OPF problem is highly data-dependent.%in essence, is equivalent to mimic a high-dimensional mapping the load inputs and optimal variable outputs.  %\textbf{First}, how can complex and massive features be efficiently filtered out and modeled in neural networks? 
\begin{comment}
In future work, we plan to explore the following aspects:
\begin{itemize}
    \item \textbf{Larger power gird networks.} We plan to explore the efficacy of this framework on much larger networks (i.e., thousands of buses), and using learning to solve computationally intense, such as security constrained AC-OPF problems on faster timescales.
    \item \textbf{A Generative Adversarial Network(GAN) model.} We propose to adopt a generative adversarial model for generating false solutions and use discriminative networks to tell whether a given solution is feasible or not. The discriminative network plays a role to help experts quickly decide whether a solution is good enough.
    \item \textbf{Exploiting benefits from active sets.}  Learning the active set of constraints at optimality has been shown to significantly simplify~\cite{misra2018learning,baker2019learning,deka2019learning}. We plan to exploit the benefits of active sets to reduce the computation complexity and facilitate the efficiency of learning model.  
\end{itemize}
\end{comment}

\subsection{Model selection}
\label{sec4-2}
%During the model construction phase, we consider several different methods of model construction: 1) several separate models for each output variable, i.e., $V_a, V_m, P_g, Q_g, Z, \lambda$ and $\mu$;
%2) a concatenate model to predict all variables.
%3) a multitask learning model to predict all variables but has some specific layers to each output variable.

To optimize a particular metric, we generally train a single model or an ensemble of models to perform our desired task. So, we design model type \uppercase\expandafter{\romannumeral1} (i.e., several separate models) for each output variable i.e., $V_a, V_m, P_g, Q_g, Z, \lambda$ and $\mu$ and model type \uppercase\expandafter{\romannumeral2} (i.e., an ensemble model) to predict all variables but shares all layers to each output variable.

During the training phase of model type \uppercase\expandafter{\romannumeral1}, we fine-tune and tweak these models until their performance no longer increases.
While we can generally achieve acceptable performance in this way, by being laser-focused on our single task, we ignore information that might help us do even better on the metric we care about.
Like the observations of Sec~\ref{sec4-1}, output variables have strong ties, which are ignored in model type \uppercase\expandafter{\romannumeral1}.
Specifically, this related information comes from different models that cannot be shared with each other.
Meanwhile, the ensemble model shares information and predicts all variables but lose a tailored design for each variable.
These different variables stand for different physical meanings in power grid simulation.
Hence, we design model type \uppercase\expandafter{\romannumeral3}, a Multi-Task Learning (MTL) model. 
By sharing representations between related tasks, we can enhance our model to perceive useful information from shared layers and also develop a better specification for each task. The details of MTL construction are discussed in Sec~\ref{sec5-4}. 



%\textcolor{wq}{1 page}

%\textcolor{wq}{How to design the experiments here and do not show the roof line model?}

%In scientific applications, there are several challenges to address for developing the neural network based approximation.

% First, how to choose the inputs and outputs for the neural network model?
% Different input signals may have different impact on generating the targets. 
% \textcolor{red}{add more.}

% Second, how to guarantee the robustness of neural network model?
% How to provide a good initial solution to the ACOPF  problem by learning-based approach?
% %
% Due to the nonlinear and non-convex nature of the ACOPF problem, finding a solution with a conventional iterative method may fail to converge.
% %
% Using warm start initialization can mitigate failure rate and help ensure convergence. However, For each case, (1) obtaining a high-quality initial point requires highly extra and unique computational time; (2) there is no systematic way to get a good initial point for the current situation.
% First, the algorithms should be able to solve non-convex AC-OPF problems reliably, even when an initialization is located far away from a local minimum.
% However, the neural networks mostly provide an approximate model of the physical constraints, which may result in solutions that violate important system constraints.

% Third, how to develop a systematic approach to guide the design of the approximate model?
% Most existing methods adopt heuristic designs of models.
% %

% Second, they should converge sufficiently fast and exchange as little information as possible.



% There are several research challenges for the design of learning-based start. 
% %
 
% %

% %
% Third, they should comprise a low-complexity coordination step (ideally based on neighbor-to-neighbor communication). 


%Furthermore, it is desirable to allow considering problem partitions related to “operational practice” to mirror the actual Transmission System Operators (TSOs) regulation zones \cite{faulwasser2018optimal,baker2019learning}.%In scientific applications, the dataset is complex and high-dimensional. %Generally, filtering out unuseful dataset can reduce the inference overhead of neural network model, and also improve model efficiency.%Generally, predicting fewer variables will reduce the complexity of model topology and improve prediction accuracy.%Our goal is to use the most essential variables to maximize model efficiency and achieve good speedup. %\textcolor{gk}{what performance? speedup, accurancy of the NN model, etc. it might be confusing.}.%, we also include these variables as potential output features candidates. %\textcolor{gk}{candiate pool for variables?}. 
%
%We use eight different input problems as our test cases and generate $10,000$ samples with various input loads as test samples to analysis each component.%For example, $X$ is a factor with a user-defined initial value involved in a solving procedure.
%If the factor $X$ is initialized with the ground-truth value, then the execution time of convergence process is dramatically reduced, leading to a high success rate and high speedup, so we recognize that factor $x$ is a critical variable.%For example, we can have rough $X$ and precise $\lambda$, $\mu$ and $Z$ as input signal to the solver.
%% We propose to experiment on the following combinations as initial value:
% \begin{enumerate}
%     \item only using the rough data source of $(X, Z, \lambda, \mu)$;
%     \item only using the precise data source of $(X, Z, \lambda, \mu)$;
%     \item using the combination of rough and precise data source.
% \end{enumerate}
%We show all combinations in Table \ref{tab:Ablation}. 
%

\begin{comment}
\begin{itemize}
    \item\textbf{Observation 1}: $Z$ has strong reliance on $\mu$ and $\lambda$. In Lagrangian multipliers, if we only initialize the solver with precise data of Z, the success rate is pretty low, observing from cases \uppercase\expandafter{\romannumeral2} and \uppercase\expandafter{\romannumeral10}); Also,  if we initialize with a precise $Z$ and one precise variable ($\mu$ or $\lambda$), the solving process is still fragile, observing from cases \uppercase\expandafter{\romannumeral4}, \uppercase\expandafter{\romannumeral6}, \uppercase\expandafter{\romannumeral12} and \uppercase\expandafter{\romannumeral14}). 
\item \textbf{Observation 2}: $\lambda$ is strong independent. Only starting with a precise $\lambda$, the solving process enable achieve a $100\%$ success rate, observing from cases \uppercase\expandafter{\romannumeral5} and \uppercase\expandafter{\romannumeral13}. Once involving another multiplier ($\mu$ or $Z$), the solving process can not always achieve $100\%$ the success rate, observing from \uppercase\expandafter{\romannumeral6}, \uppercase\expandafter{\romannumeral7}, \uppercase\expandafter{\romannumeral14} and \uppercase\expandafter{\romannumeral15}).  
    \item \textbf{Observation 3}: Only starting with a precise $X$ (case \uppercase\expandafter{\romannumeral9}) or only starting with all precise Lagrangian multipliers (case \uppercase\expandafter{\romannumeral8}) can not guarantee 100\% success rate.
    
\end{itemize}
%\textcolor{gk}{Let's make sure that we always use either capital or lower cases for variables.}%\textcolor{wq}{To be continue... all 16 scenarios.}
\end{comment}%Although incorporating equality multiplier can provide $100\%$ success rate without the disturbing of $\mu$ and $Z$, the speedup is still not greatly improved. 

%A good trade-off between performance and success-rate is XXX.%Based on our precision rounding method, we conduct an exhaust search on possible directions. % The details of multitask model will be discussed in Sec~\ref{multitask}.
%For model morphism, we evolve its topology and improve model accuracy with two operations,
%We adopt a precision rounding method to simulate the precision of model outputs and analyze its impacts on success rate and speedup.
%Then, we analysis the sensitivity of search space with different improved cases using mantissa rounding. The search space includes four variables ($X$, $\lambda$, $\mu$, $Z$) and each variable has a knob if the variable should improve its precision. In total, there are $2^4$ combinations.
%To validate the sensitivity of each direction, we use the precision rounding value of ground truth to represent these combinations. 
%Here, we introduce the precision rounding method:
%\begin{equation}
%    \hat{x} =\round{\frac{x}{RP}}\cdot RP,
%\end{equation}
%where $x$ represent the ground truth, $RP$ is the factor of rounding precision. Rounding factor $RP$ decide how much the mantissa to be cut off. 
%A smaller RP leads to higher precision loss. For example, processing with the rounding factor $1e2$, the original data $123.45678$ only keep the first two mantissa, i.e., $123.45$. While, processing with the rounding factor $1e4$, the original data can keep more mantissa, i.e., $123.4567$.


%Auto-Keras~\cite{jin2018auto} is an open-source software library for automated machine learning (AutoML). It is developed by DATA Lab at Texas A\&M University and community contributors. Auto-Keras provides functions to search for architecture and hyperparameters of deep learning models automatically. The main difference between using
%Auto-Keras comparing with the AutoML systems lies at shallow models is the much longer time consumption since a number of deep neural networks are trained during the neural architecture search. A typical workflow for the Auto-Keras system is as follows~\cite{naeini2019transfer}. (1) A user calls the API. (2) The Searcher generates neural architectures on the CPU. (3) The graph builds real neural networks with parameters on RAM from the neural architectures. (4) The neural network is copied to GPU for training. (5) Trained neural networks are saved on storage devices \cite{jin2019auto}.


%Auto-Keras is quite useful for generating and filter out the most efficient models in terms of model accuracy. However, it mainly focuses on image regression and classification, which is a little different from our target, scientific computation. Hence, the code is modified by 1) adding the consideration of execution time instead of only considering the accuracy; 2) extend the code to enable input/output the scientific format(matrix usually) instead of images.

%, implemented in pure-Matlab.%Several available OPF solvers are provided to solve large-scale AC- and DC-OPF problems.
%This solver has been applied to general nonlinear optimization problems outside of Matpower and comes with a convenience wrapper function to make it trivial to set up and solve linear programming (LP) and quadratic programming (QP) problems. %Note selecting PARDISO as the linear solver can often dramatically improve both computation time and memory use when solving large-scale AC-OPF problems with MIPS.
%\textcolor{wq}{add an evidence to show it is reasonable.}
%We take the IEEE 30-bus system in Matpower as an example to explain the process of sample generation. 
%The IEEE-30 bus system contains 30 buses, six generators, and 40 connect lines.


	    %These existing work are unsatisfying due to that there are no include all the inputs of AC problem and can not guarantee that the predicted solution is optimal.
%In our task, our fundamental purpose is to estimate a plausible solution to the power grid using neural networks.
%
%And the existing solver is to perform numerical optimization on the equations (??).
%
%In order to estimate a plausible solution to the power grid using neural networks, many research \cite{ng2018statistical} devote to learn a mapping between the input power requirement and the output dispatch scheme.
%
%Pan et al~\cite{pan2019deepopf} recently propose a DeepOPF method that use MLP to learn such mapping and apply it to obtain optimized operating decisions upon arbitrary load inputs.
%

%~\textcolor{wq}{???} 
%because~\textcolor{wq}{AC problem is non-convex while DC is convex}.
%
%Ahmed et al~\cite{zamzam2019learning} develop an online method that leverages machine learning to obtain feasible solutions to the AC problem by loading the optimal generator set-points and enforcing generation limits. However, AC grid contains more voltage phase angles beyond magnitudes %and reactive parts of power generation. These existing work are unsatisfying due to that there are no include all the inputs of AC problem and can not guarantee that the predicted solution is optimal.
%
%We also conduct experiments on AC problem according to their settings for DC counterparts.
%
%\textcolor{gk}{there are also other work to cite}  \cite{zamzam2019learning, ng2018statistical}.
%

%\noindent\textbf{Applying neural networks to HPC applications.}%Richard et al.~\cite{richard2014artificial} leverage a neural network to predict the evolution of the pulsed heat load during plasma operation of the simulation process. %In this work, we use neural network models to modelling computation for a representative HPC application. 
%\textcolor{gk}{i wouldn't use "approximation" for our work, "modelling" is a better term}% \textcolor{gk}{why do we give a reference to  \cite{tompson2017accelerating} for existing work? we didn't even describe this work}
%make the whole process faster.
%\textcolor{gk}{also incorporating hard and soft contraints, use of multi-task model and notable speedup}

%\noindent\textbf{Multi-task Learning.}%
%Their model learns common latent features and exploits the synergy
%among the tasks which boosts up their individual performances.
%%, given a sentence, outputs multiple language processing predictions: 1) part-of-speech tags, 2) chunks, 3) named entity tags, 4) semantic roles, 5) semantically similar words and 6) the likelihood that the sentence makes sense.
%
%All the tasks use labeled data except the language model which is learnt from unlabeled text and represents a novel form of semi-supervised learning for the shared tasks. 
%In this paper, to take full advantage of the connections between the outputs of multi-task learning, we generate a more precise warm-start point to reduce the number of subsequent iterations.
 %\textcolor{gk}{%
%Using multi-task learning to simultaneously generate the warm-start point and the intermediate Lagrangian multipliers is beneficial to the improvement of accuracy~\textcolor{wq}{XXX}.\section{Background}
\label{sec2}
\textcolor{wq}{1 page}

\textcolor{wq}{\subsection{Neural Network-based approximation ??? or Scientific Machine learning???}}
\textcolor{wq}{Need rephrase.}
Machine learning has made great progress in recent years, achieving state-of-the-art results on many scientific applications including computer vision, natural language processing, robotics, etc.
For numerical computation problems, machine learning enables discover behaviors, fetch characteristics, train and build a corresponding model to accelerate High performance computing (HPC) applictions.
There are two main tendencies of implementing machine learning in HPC field. One is using machine learning to generate more output data for accuracy or steering simulation between successive iterations through refining the network model to producing more accurate data that efficiently converge in the next iterations. 
The other one is replacing numerical simulation models with machine learning approximation.
medicine~\cite{Medicine}.
Racah et al.~\cite{racah2017extremeweather} presented a multichannel spatiotemporal CNN architecture for prediction and data analysis of extreme weather events.
Candle~\cite{candle.cels} uses semi-supervised machine learning to automatically read and encode millions of clinical reports into a form that can be computed upon. These encoded reports will be used by the national cancer surveillance program to understand the broad impact of cancer treatment practices and drive simulations of entire cancer populations to determine optimal treatment strategies for patient cohorts.

%\textcolor{wq}{Need more attractive introduction.}

%In particular, the current methodology is rather ad-hoc and application-specific. There is no systematic and principled approach to enable general application of machine learning methods to scientific simulations. 
%The lack of a systematic and principled approach is especially problematic to ensure high simulation quality when using machine learning.  Furthermore, using machine learning requires domain scientists to have machine learning knowledge, while they usually do not have sufficient machine learning background. How to make machine learning techniques widely accessible and usable to domain scientists is largely unexplored. %In this thesis, we focus on some fundamental limitations in using neural network-based approximation to accelerate HPC applications.

% Existing work shows that neural network can be used to approximate code regions for applications in diverse domains~\cite{micro2012neural,Esmaeilzadeh:2012:ASD:2150976.2151008,carleo2017solving,mlfft,md_ml17}.  
% In this paper, we also use the neural network to replace computation- or memory-intensive code regions. We briefly review the neural network as follows.
% A neural network is composed of nodes (i.e., neurons) and edges. 
% Nodes are organized into layers of a neural network; nodes across layers are connected by edges; each edge has a weight. 
% We learn the optimal weights when training the neural network. 
% %that the adjusts in the learning process. 
% Typically, there are three types of layers: the input layer, the hidden layer, and the output layer. 
% A node of an input layer accepts input data of the neural network. 
% A node of a hidden/output layer is the weighted sum of the input data.
% An output layer is responsible for generating the desired results.
% % it depends on whether the neural network is for a classification problem or a regression problem. 
% Besides, there are bias nodes at each layer, which are used for compromising noise in the input data to avoid overfitting. 
% There can be an activation function such as sigmoid or ReLU for a layer to rectify the incoming data for the next layer. 

% In our work, we use supervised learning to replace computation in HPC applications with neural networks, i.e., MLP (Multilayer Perceptron). 


\subsection{OPF and AC-OPF}
\textcolor{wq}{ Need rephrase.}

There are several research challenges for the design of distributed AC-OPF algorithms. First, the algorithms should be able to solve non-convex AC-OPF problems reliably, even when initialized far from a local minimum. Second, they should converge sufficiently fast and exchange as little information as possible. Third, they should comprise a low-complexity coordination step (ideally based on neighbor-to-neighbor communication). Furthermore, it is desirable to allow considering problem partitions related to “operational practice” to mirror the actual Transmission System Operators (TSOs) regulation zones \cite{faulwasser2018optimal,baker2019learning}.



\subsection{Multi-task Learning}



Multi-task learning aims to simultaneously obtain the inference results for multiple tasks that are used to be solved separately with different neural network models.
%
Multi-task learning models typically composes of shared layers and task-specific layers.
%
The shared layers are responsible for extracting common features for different tasks.
%
While the task-specific layer will borrow the information from those common features to generate their own dedicated results.
%
Compared to multiple separate models for each task, the multi-task learning mechanism enjoys reduced model parameters via weight-sharing.
%
Furthermore, multi-task learning is helpful for reducing the inductive bias that may occur in each individual task~\cite{?}.
%


%
For example,  Ranjan~et al.~\cite{Ranjan2019HyperFace} propose a multi-task model for face detection, landmarks localization, pose estimation and gender recognition.
%
Their model learns common latent features and exploits the synergy
among the tasks which boosts up their individual performances.
%
In the natural language processing,  Collobert et al.~\cite{collobert2008unified} describe a single language model that, given a sentence, outputs multiple language processing predictions: 1) part-of-speech tags, 2) chunks, 3) named entity tags, 4) semantic roles, 5) semantically similar words and 6) the likelihood that the sentence makes sense.
%
%All the tasks use labeled data except the language model which is learnt from unlabeled text and represents a novel form of semi-supervised learning for the shared tasks. 
In our task, our fundamental purpose is to estimate a plausible solution to the power grid using neural networks.
%
Using multi-task learning to simultaneously generate the warm-start point and the intermediate Lagrangian multipliers is beneficial to the improvement of accuracy~\textcolor{wq}{XXX}.
%

%And the existing solver is to perform numerical optimization on the equations (??).
%
%Hence, a straightforward method is to learn a mapping between the input power requirement and the output dispatch scheme.
%
%However, according to our experiment, the~\textcolor{wq}{xxx}.
%
%%\textcolor{gk}{it would be great if we can come out with a name for our work}
%Smart-PGSim
%The framework of using a neural network to accelerate AC-OPF is divided into the training and inference stages. We first construct and train a DNN, i.e., a multitask learning model, to learn the mapping between the load inputs and the power generations and bus voltage outputs. We also directly predict factors $Z, \mu, \lambda$, which show tight ties with $X$. The training process is conducted offline. Then, the DNN model can be used for online prediction. In the inference stage, we directly apply the learning model to solve the AC-OPF problem with given load inputs.  This is different from recent learning-based approaches for solving (AC-)OPF, where machine learning only helps to facilitate existing solvers, e.g., by identifying the active constraints~\cite{deka2019learning, ng2018statistical}.  Specifically,  We will discuss how to incorporate the equality constraints and inequality constraints as soft constraints in Section~\ref{sec6:soft_constraints}. %The detail of sensitivity study is discussed in 
%The Smart-PGSim framework consists of three main modules: offline sensitivity study (), the multitask model , and physics informed learning (. Their relationships are depicted in Figure~\ref{fig:overview}. We explain them in detail as follows.%\textcolor{wq}{why not acceleration?}.%Generally, predicting variables at low precision will reduce the complexity and overhead of model and improve accuracy.
%\textcolor{wq}{When we use neural networks to predict and replace variables in scientific applications, low-precise prediction decreases the success rate of simulation and even causes a crash. }% \textcolor{gk}{Table 1 names different inputs as bus 5,9,..300. That is not completely true. I guess you mean IEEE 30-bus test case - which consists of 30 buses, 6 generators, 41 branches and 20 loads. 
%  	Maybe we should call them "case" rather than "bus". But we should be careful for this as well. Because in Table 1, each row is also a test-case for us.
%  	And I could not find any table that shows the characteristics of each test case. 
%  	 Do you think we should have them? If we don't have space, maybe we should give a reference for their properties.
%     I just checked from other papers - they mainly use "test systems" for different input cases} %\textcolor{wq}{gk:let's use another word not to confuse power grid engineers. wq: use ``cases'' instead of scenarios.} %In the AC-OPF problem, the electricity generation model minimizes cost based on generation constraints, line flow constraints, and bus voltage constraints. The main drawback behind current neural network model is that these "black-box" methods do not exploit the physical meaning of the power flow and structure of the AC-OPF problem. Physical understanding should be incorporated as the bedrock of modeling, such as the right range of variables, application constraints, and physical laws. Incorporating these constraints into our neural network model not only facilitates the efficiency but also enables quality guarantee of power grid simulation. We allow the user to enforce hard and soft constraints during the model construction.

%\textcolor{dong}{%facilitates the efficiency, \textcolor{red}{(what does it mean by "facilitate efficiency"? What is "efficiency"?)} but also enables quality guarantee of power grid simulation \textcolor{red}{(we can enable quality guarantee?)}. }  
%\textcolor{dong}{}%\textcolor{red}{(I don't understand why the ground-truth data needs to be normalized.}\textcolor{wq}{ because  we need to use ground truth guide the training of outputs.)}
%}

%\textcolor{dong}{We also incorporate hard constraints during the prediction phase. \textcolor{red}{(give some details here)}}

%We can incorporate hard constraints in neural network models during the training phase and the prediction phase. Incorporating constraints during training generally makes maximal use of training data by adding non-linear activation function at the last hidden layer. There are also additional opportunities to employ constraints at the time of prediction by projecting predictions onto the region induced by the constraints.

%\textcolor{gk}{there is only one hard contraint on Z, so we could remove the bold text - Hard bound on auxiliary task.}
%\textbf{Hard bound on auxiliary task $Z$.} 
%In Eqn~\ref{eqn:largran}, we observe that the equation is satisfied with a condition of Lagrangian multiplier $Z>0$. During model training phase, we first normalize the ground-truth data $Z$ rescaled to the range $[0,1]$, then apply a ``Sigmoid'' activation function at the last layer to bound the output range. This hard bound operation enforce the outputs hit on the a valid range. Once the model is well-trained, the restricted prediction incorporating the variable constraints greatly improves model feasibility without violation. %The soft constraint includes the domain knowledge that can be used to improve model efficiency, such as physical principles, conservation laws, and other priors gained from theoretical or computational studies.
%To incorporate soft constraints, we modify the loss function used in training through involving application-specific knowledge. It is understood that the loss function selection is guided by the task and data, and the loss function design also impacts the solvability and generalizability of proposed model. Therefore, opportunities exist for developing loss functions to incorporate application knowledge. 

%In AC-OPF problem, we incorporate application specific information through involving the following soft constraints.

%\textcolor{gk}{define L1 loss}%}\textcolor{red}{(put the definition of L1 loss into the background section.)}
%Guaranteeing the power flow equality constraints, i.e., Eqn~\ref{eq:1b} is enable to keep the power grid system stable and predict a feasible solution. We encapsulate this equality constraints ($Loss_{eqn}$) as $L_1$ loss, i.e., the absolute loss, in loss function to guide model training.   
%Incorporating the equality and inequality constraints minimize the loss of optimization vector $X$ between model prediction and the ground-truth, and also facilitate the robustness of the predicted solution through implying the physical law. 

%\textcolor{red}{(The following paragraph can be deleted, if we don't have space.)}\textcolor{red}{(did we incorporate the inequality constraints?)}
%\textcolor{dong}{%\textcolor{gk}{what about "The Optimal Power Flow Problem" as a title?}

%\textcolor{gk}{I think related work should be before this section, then we can briefly descripe OPF, ED, etc... Then, in this section, we can directly go to the problem formalation of AC-OPF.}

 %The power grid simulation, in essence, solves the optimal power flow (OPF) problem. In general, the OPF problem can be divided into three categorites: Economic Dispatch (ED), Direct Current (DC-)OPF, and Alternating Current (AC-)OPF problems \cite{christie2000transmission}.
%\textcolor{wq}{Wenqian: Add brief introduction to quickly explain the difference between three problems.} 
%The AC-OPF, being the most widely applied one, is non-convex and most challenging to deal with.  \textcolor{dong}{We focus on the AC-OPF in this paper.}
%\textcolor{gk}{do we plan to introduce OPF problem formulation? If so, we can add it here before introducing AC-OPF.}%\subsection{Problem formulation for AC-OPF}

%\textcolor{gk}{what about "Problem formulation for AC-OPF" as a title?}%Hence the gradient is small.
%\begin{enumerate}
%    \item In ground-truth dataset, there is few variables in $X$ reaches the minimal and maximal and the majority distributes in a relatively small central range. Normalizing $X$ with the boundaries $a_i$ and $b_i$ expands the prediction range and decreases the prediction accuracy. For example, the bound range of $P_g$ at the 92-th bus is [0, 390] in IEEE-300 bus system. While, the ground truth only varies from 294 to 339 with different power loads.
%    \item After normalization, the difference is weaken.  Normalizing rescales the original range into range [0,1] through simple linear transformation.  Most variables in $X$ have a larger range, for example the value range of $P_g$ is [0, 2030]. Mapping the large range to the small range through the simple linear transformation decreases the diversity of samples, and lost some invisible information. 
%    \item  After normalization, inputs will be regularized as the same outputs in deep neural network. There exist a gradient vanishing problem in our model after using normalization and deep layers. 
%\end{enumerate}

%\textcolor{gk}{i guess it is equality and inequality loss function}%To minimize the error of cost prediction, we use L1 loss of the predicted cost \textcolor{dong}{as the optimization target} to improve model accuracy. \textcolor{red}{(please verify if the above sentence is correct.)}
%The final goal of the AC-OPF is minimizing the objective function $f(X)$. We use the default objective function in Matpower, i.e., quadratic cost function $f(X) = X^\intercal Q X + C^\intercal X +k$. To minimizing the error of cost prediction, we add L1 loss of predicted cost to improve model accuracy. %\textcolor{wq}{1.5 pages}

%In this section, we discuss the generation of training data for the MTL, training of the MTL, and how the overall feasible solution to the AC OPF problem is obtained.%tasks \textcolor{red}{(do we define ``tasks'' somewhere?)}. 
%\textcolor{dong}{%}

%the multi-task learning mechanism enjoys exchanged information from shared layers and specializes dedicated design for task-specific layers. 
%Multi-task learning is a inductive transfer learning mechanism, in which typically composes of shared layers and task-specific layers. The shared presentation layers make several related tasks better combine related information, while the task-specific layers separately exploit the task specific information. %\textcolor{red}{(In the above paragraph, what are the main task and related tasks?)}
%\textcolor{gk}{in the following text, we use "axiliary task" as a related task. we should always use the same term }


%\textbf{Shared representation in shallow layers.}%\item Parameter sharing. The multi-task learning model takes several shared layers in shallow layers as common layers. These common layers share the same weights and topology design.  Through sharing parameters, tasks share low-level semantic information to complement domain knowledge with related tasks. Meanwhile, hard parameter sharing greatly helps alleviate risks of overfitting. The noise brought by sharing can improves model generalization. Furthermore, the multi-task learning model helps reduce the computation overhead comparing training multiple tasks with seperate models.
    %While the local minimal of different tasks are in different positions in multi-task learning. With incorporating multiple losses, the multi-task learning model is optimized by multiple principles. Also, the interaction between different tasks could effectively help the model to escape from the local minimal. %Multi-task learning model exploit and interact useful information in shared layers, then attention focusing on task-specific layers to specialize each task. In task-specific layers, we delicately design specific model topology for each task based on their attributions and demands. For example, as a requirement of the output of task ``A'' should be positive, we can add ``ReLU'' activation function at the last layer  to bound the output range in task ``A''. 
%Although multi-task learning has been showcased to achieve good performance on various fields~\cite{ref}, multi-task learning in large-scale complex info and data still faces a range of challenges of feature selection~\cite{ref}. Not only reducing data complexity in high-dimensional, noisy, and uncertain input data but also keeping the validity of efficient tasks is critical in model construction.

%\textcolor{red}{(the following discussion has nothing to do with the loss function. Maybe we should delete it.)}


%\textcolor{red}{(The following assumptions may be placed into the background section. )}
%Based on the assumption that the AC-OPF problem of a power network is repeatedly solved, a well-proposed model can be frequently used without consideration of training overhead. In each power gird system, the configuration of power network topology is fixed, i.e., the numbers of  generators and buses are known factors to the power network. %\textcolor{red}{(what is the last part?)}%the real reason behind this is the parameter $\gamma$ approaches to zero. \textcolor{red}{(re-write the above sentence)}%\textcolor{red}{($Loss_{f(x)}$ and $Loss_{Lag}$ are soft constraints or not?)} 
%We leave the study of weight importance as our future work.  \textcolor{red}{(where is the weighted sum? Can you use an equation to show it? We cannot say the "study of weight importance as future work", because it is too lame...)}

%\textcolor{red}{(the below paragraph can be deleted, if we don't have enough space.)}%\textcolor{wq}{wq: pending... different models with different loss.}

%The training objectives  components; e.g., regularization terms that can encapsulate soft constraints, and these components usually are composed in a weighted sum.%
%Their model learns common latent features and exploits the synergy
%among the tasks which boosts up their individual performances.
%%
%Using multi-task learning to simultaneously generate the warm-start point and the intermediate Lagrangian multipliers is beneficial to the improvement of accuracy~\textcolor{wq}{XXX}.%The power loads, which is the only varying factor,  are decided by user demands. Hence, we only take the power loads at each bus (both the active parts $P_d$ and reactive parts $Q_d$) as inputs of multi-task learning model and we design the high-tailored model for each power network. As discussed in Section~\ref{sec2}, we take the problem solution as the main task in model outputs and argument the Lagrangian multiplier as auxiliary tasks.   
%\textbf{Auxiliary tasks.} We extend model outputs with auxiliary tasks. As mentioned in Section~\ref{interior_point_solver}, Lagrangian multipliers, i.e., $\lambda$, $\mu$ and $z$ are estimated to facilitate the final convergence. \textcolor{wq}{wq: add sensitivity study evidence here.}  In our multi-task model design, we collect these features for estimating  $\lambda$, $\mu$ and $z$  as an augmentation to  provide additional features for main tasks. Through ``eavesdropping'' the auxiliary tasks, the main tasks can interact with relevant tasks implicitly. %a set of essential variables, i.e., $X,  \lambda, \mu, Z$. The optimization variables $x$ include four parts, $V_a$, $V_m$, $P_g$ and $Q_g$. In total, we infer seven variables. In this way, we not only include the solution variables $X$ but also predict the key factors, i.e., Lagrange multipliers $Z, \lambda, \mu$ that impact the converge rate. In contrast these multipliers are not included in existing learning-based approaches for AC-OPF problem.

%\textcolor{gk}{for optimal power flow} \cite{pan2019deepopf,zamzam2019learning, ng2018statistical}.
%Here, we take the IEEE 300-bus system as an example to show the model construction. As shown in Fig \ref{fig:MTL}, the shared representative in shallow layers first take electricity loads $P_d$ and $Q_d$ at each bus as inputs, which are $2 \times n_b$ ($n_b$: number of buses) vectors. In our case, it takes $2\times300$ features as inputs. In the 300-bus case, there are five fully-connected networks in the shared layers. The corresponding node numbers are $600, 720, 840, 960, 1080$. Later, the extracted shared features are fed to multiple estimators for generating more specialized outputs. Each estimator is task-specific. For example, the $V_a$ estimator aims to predict the $V_a$ variable. In general cases, all these seven task-specific estimators have their specific network architecture for the task-specific layers. The task-specific layers are designed with different numbers of layers, neurons, and different activation functions according to different outputs. 
%We list all the network configurations for the used estimators of the seven variables in Table ~\ref{tab:model_config}. For example, for $V_a$, our $V_a$ estimator consists of 4 full connected layers, where there are $880, 680, 480 , 300$ neurons for each corresponding layer. We use ReLU for all layers except the last one to increase the nonlinearity of our neural network.
%We impose a variant of $L_1$ loss (i.e., Charbonnier loss) between each of the predicted output variables $v$ and the corresponding ground-truth values $v_{gt}$ collected by MIPS solver. The Charbonnier loss is given by:%The observation in Sec xxx \textcolor{wq}{(add sensitivity study evidence here)} shows that factors $X,Z,\lambda,\mu$ are highly  correlated, so we feed all these factors into a comprehensive model.   %\textcolor{red}{(adding one or two sentences here to explain why the difference is a problem for modeling.)}
%\textcolor{dong}{We rescale the values of the four variables into the range of [0,1], using the following equation.
%}%Data pre-processing is a data mining technique that involves transforming raw data into an more efficient format so that the networks will focus on learning the intrinsic mapping between input and output signals. The two most discussed pre-processing methods are normalization and standardization.%\textcolor{dong}{We rescale \textcolor{red}{xxxxxx} to have a mean ($\mu$) of 0 and a standard deviation ($\sigma$) of 1 as follows.}%\textcolor{red}{(did we mention "regularization" somewhere before this section?)}

%\textcolor{red}{(Is the following paragraph for post-processing? Re-write this paragraph. It's confusing.)}
%After generating the outputs in the learning model, we back forward the outputs to original format. For examples, using normalization as pre-processing, we back forward the predicted variable $\overline{{x}^{\prime}}$ with historic data $x_{min}$ and $x_{min}$ of the pre-processing phrase. 

%\textcolor{dong}{%\textcolor{gk}{I just wonder if we need to talk about Matpower under problem formulation. The MISP solver is one of the solvers used to solve the Newton linear system?}%this equality constrained problem \textcolor{red}{(which equality constrained problem? $H(X)+Z=0$?)} is as follows. 

%Matpower performs power grid simulation with the primal-dual interior point solver called Matlab Interior Point Solver (MIPS). To solve the AC-OPF problem, the solver converts the inequality constraints in Eqn.~(\ref{eq:1c}) into equality constraints using a barrier function and vector of positive slack variables $Z$, i.e., $H(X)+Z=0$. Given value of $\gamma$, the Lagrangian for this equality constrained problem is
%\textcolor{red}{(what is the original problem?)}. 
%where $\gamma$ is the perturbation parameter and the solution to this problem equals to that of the original problem if $\gamma=0$. % \textcolor{red}{(the following formulation means the conditions are satisfied? What is F() and $\mu$ in the following equation?)} \textbf{% (1) computing $\Delta X$ and $\Delta \lambda$ to update $X$ and $\lambda$: 
% \begin{equation}
%   X \leftarrow X + \Delta X,\\
% \lambda \leftarrow \lambda + \Delta \lambda; 
% \end{equation}


% (2) computing $\Delta Z$ based on $\Delta X$ and update $Z$:

% (3) computing $\Delta \mu$ based on $\Delta X$ and $\Delta Z$.



%In each Newton step, the computation steps follows the order of 1) compute $\Delta X$ and $\Delta \lambda$; 2) compute $\Delta Z$ based on $\Delta X$; 3) compute $\Delta \mu$ based on $\Delta X$ and $\Delta Z$. 

%where $F_x$ donates the first derivatives, e.g., $F_x = \frac{\partial F}{\partial x}.$  
%Given an initial value, MIPS iteratively converge to find the optimal.%}
%The process of solving the Largrangian equation in Matpower is based on Newton method, which involves large computation overhead that iteratively converges to meet convergence criteria. The Newton update step can be written as:}%In this paper, we propose using a multitask learning model to accelerate the solving process of AC-OPF problem in powergrid simulation. We use pre-processing technology to rescale the data distribution, which achieves better performance on model training. Our experiments show that the developed MTL model achieves $1.49\times$ speedup than the original numerical method.
 %Using machine learning (especially neural networks) to approximate computation in HPC applications and improve performance has shown preliminary success recently. However, using this approach faces fundamental limitations due to the lack of model flexibility and generality. In this paper, we focus on a specific HPC application and introduce a systematic approach to address the above limitation. In particular, we introduce a framework (Smart-fluidnet) that automatically uses multiple neural network models at runtime to approximate computation and make best efforts to meet the user requirements on simulation quality and execution time. The framework includes a series of techniques to construct and select neural network models. 
%Based on the comprehensive evaluation, we show that Smart-fluidnet is $1.46\times$ and $590\times$ faster than a state-of-the-art neural network model and the original fluid simulation respectively on an NVIDIA Pascal GPU, while providing better simulation quality than the state-of-the-art model.

%%
%% The next two lines define the bibliography style to be used, and
%% the bibliography file.
%\bibliographystyle{ACM-Reference-Format}
%\bibliographystyle{plain}
%\textcolor{gk}{if we need to cut, we can trim a little this paragraph, I believe we don't need to go to the details of each approach}% For example, scientists working to detect neutrinos at Fermi National lab have realized a 33\% improvement in neutrinos detection using a convolutional neural network~\cite{ichep16:radovic};  
% Scientists achieve Bose-Einstein Condensates state in only 10-12 experiments using neural networks instead of 140 experiences using traditional models, which reduces the simulation time by 10 times~\cite{sr15:widley}. 
% Other successful examples of using neural networks for HPC include recognizing extreme weather events in large-scale climate simulations at Lawrence Berkeley National Lab (LBNL)~\cite{nips17:racha}, and precision medicine for cancer~\cite{candle_anl} at Argonne National Lab. 
%The basic optimal power flow is an electricity generation model to minimize cost with generation constraints, line flow constraints, and bus voltage constraints.%For example, the entire Illinois power grid system~\cite{chiang2016large} comprises of 2522 lines, 1908 nodes, 870 demand points and 225 generator points. %due to high callback \textcolor{red}{(what is callback?)}
%%Recent neural network approaches for solving (AC-)OPF only helps to generate an approximate solution~\cite{guha2019machine, baker2019learning, zamzam2019learning} or facilitate existing solvers, e.g., by identifying the active constraints~\cite{deka2019learning, ng2018statistical}. 
%\textcolor{red}{(what is the limitation of existing efforts?)} 
%%However, their methods cannot provide the optimality for the solution because we know that neural work is only trying to \textit{approximate} the optimal solution.

%These tight latency requirements and large system sizes make power-grid simulation a computational challenge task.
%\textcolor{gk}{ gk: add the importance of the power grid sim.}

%Recently, interest in Neural Network (NN) approaches for science and engineering has increased rapidly~\cite{KK}. %This growing enthusiasm for Scientific Machine Learning (SciML) stems from the combined development and use of efficient data analysis algorithms; massive amounts of data available from scientific instruments, scientific computations, and other sources; advances in high-performance computing; and the successes reported by industry, academia, and research communities~\cite{bundy2017preparing,royal2017machine}.
%NN-based techniques for model enhancement and acceleration in complex data mapping have dramatic growth in scientific applications, e.g., collecting billions of particle collisions~\cite{mustafa2017star}, simulating thousands of climate scenarios~\cite{covey2013efficient}, or observing millions of stars~\cite{najita2016maximizing}.


%\textcolor{gk}{what we propose comes very late}%%In this paper, we introduce a new method to apply neural network to the AC-OPF problem. In particular, we introduce a physics informed multitask learning model to initialize a good warm start point, which significantly facilitate the solving process. %This approach takes advantage of the fact that AC-OPF is routinely solved with varying values of power loads, thus leading to readily available historical data for neural networks to train on. Once neural network models are well constructed and trained, it can serve as an essential component to accelerate the solving process of AC-OPF in real-time efficiency. 
%%Different from the existing work, we use neural network to generate initial solutions and inject that solution to the AC-OPF solver. 


%Why?
%\textcolor{gk}{I think we should first explain what we do in this paper, then it will be easier to talk about limitations and our contribution. There are some sentences in the following paragraph - "our machine learning model" but we haven't say anything what we do.}

%\textcolor{wq}{wq: I list four challenges here. }
%We develop a multitask NN approach to approximate and accelerate the computation in the Powergrid application.

%However, there remains several significant challenges to accurate patterns in finding a solution with neural network-based approaches for AC-OPF simulation. %First, How to generate an optimal solution for the power grid simulation using neural network is a challenge. As a scientific HPC application, power grid simulation requires high quality control and only accepts the optimal solution. While, neural networks-based approaches bring uncertainty and approximation for power grid simulation. Namely, there exists possibilities that a learned solution may not satisfy the optima requirement. Quality and accuracy of the neural network model is  highly sensitive to perturbation of inputs. even with sufficient training models or the appropriated design of model topology. Small outliers in neural network model can result in drastic errors between the model outputs and true AC-OPF solution. Prior approaches~\cite{zamzam2019learning, guha2019machine} only give a approximate solution through learning the nonlinear mapping can not guarantee the quality of final solution. 


%First, how to ensure that applying neural networks to the AC-OPF simulation does not disturb the simulation robust is a challenge. This means xxxx.  Due to the non-convex and nonlinear nature of the ACOPF problem, the solving process itself is at the risk of a failed converge with the use of iterative numerical methods.  Hence, the situation becomes more serious in adopting a neural network solver due to the intrinsic uncertainty in the training datasets generated by numerical algorithms. Meanwhile, case differences in power grid simulation are usually huge and non-stationary. For example, electricity load is highly unpredictable and affected by seasonal effects, temperature, humidity, and human demands. This also brings additional challenges for neural network models to ensure the final converge at 100\% success rate.

%\textcolor{dong}{%Second, How to impose physical constraints to neural network to ensure the validness of prediction results is a challenge. Traditionally, the neural network model is manually constructed by computer scientists without domain knowledge and without the awareness of the requirements of domain scientists. Existing neural network models~\cite{zamzam2019learning, guha2019machine} for the AC-OPF problem are constructed as a black box. The main reason behind this drawback is that these "black-box" methods do not exploit the physical meaning of the power flow and structure of the AC-OPF problem. The most influential physical terms include generation constraints, line flow constraints, and bus voltage constraints. Incorporating these constraints into our machine learning model not only facilitates the efficiency of neural network models but also enables quality guarantee of power grid simulation. However, existing neural network models lack systematic approaches to model and impose existing domain knowledge in neural network models.


%\textcolor{dong}{}

%Third, there are no systematic approaches to guide topology design for HPC applications. How to construct neural networks to meet the requirements on performance (execution time) and simulation quality is challenging. Currently, domain scientists build neural networks intuitively. There is no systematic approach to help them build and apply neural networks for HPC applications. The recent work on Auto-Keras~\cite{jin2018efficient} and AutoML~\cite{escalante2019automl} aims to automatically generate a neural network model with high accuracy. However, they lack concerns on high performance (execution time), and focus on image processing or natural language processing. Hence, they are not directly usable by HPC.



%\textbf{First}, the existing methods that apply the neural networks to power grid simulation is not robust enough. 

%\textbf{Second}, the current model to apply the neural network to power grid simulation is not interpretable. 

%  how to minimize the variation of the solving process, given that 
%Therefore,  
%For a randomly given case, we cannot guarantee its execution time.
%\textbf{Third}, the current neural network method can not guarantee simulation quality. 

%\textbf{Fourth}, 

%Filtering out useful information in complex and high dimensional dataset of power grid simulation is not trivial to construct efficient input and output feature. 
%Neural network, in essence, is equivalent to mimic a high-dimensional mapping from the load inputs to the optimal variable outputs. 
%Discarding redundant and unuseful data of inputs and outputs not only reduces the computation overhead of neural network, but also improves model efficiency to better map their relationship. 
%On the opposite, involving useful data can better exploit the learning efficiency of neural network model.%In this paper, we introduce a framework ``Smart-PGsim'' to address these challenges mentioned above. Smart-PGsim has three major components. (1) It includes a tool to perform sensitivity study. The sensitivity study includes component analysis and prior analysis for addressing the robustness and systematical design correspondingly. We first quantify the sensitivity of related components with respect to simulation success rate and imposes the quantized sensitivity into the loss function for improving model robustness. Our prior analysis refers to adopting a perturbed ground truth signal to trigger the warm-start of a AC-OPF solver. After the component analysis, we conduct the \textit{prior analysis} to systematically guide the evolution of model topology.
%(2) \name  enables information sharing and customizes specific designs for multiple tasks by a multitask learning model. The multitask model generate a warm-start point to initial AC-OPF solver, which guarantees the optimality of final solution. % 
%(3) \name  also impose physics constraints in loss function with transformed equality and inequality constraints from the original problem formulations. 
%Based on the study results, the user can enable automatic construction based on component analysis and prior analysis of power grid simulation. %\item A new mechanism that analysing variable sensitivity for automatic model design. This mechanism address the fundamental limitation of model accuracy and feasibility in the existing neural network-based approximation. We demonstrate great potential of using this methodology to meet user requirements on the simulation quality and execution time.

% \begin{itemize}
% \item  We do a sensitivity study on output tasks. xxx...
% \item Development and validation of Multi-task learning architecture for modeling the solving process of power grid simulation. First demonstration of framework to construct shared representative between tasks.
% \item  We impose physical constraints to optimize the model. XXX...

% \end{itemize}

%\textcolor{gk}{Just a suggestion, I would organize the intro in this way: 1) Importance of machine learning/deep learning nowadays, 2) Use of NN in scientific computations, existing attempts, and their success story 3) introducing power grid ap and its importance in HPC 4) existing studies to leverage NN in ACOPF problem. This can be very short, just a list and a very general descirption 4) Then we can tell what we propose (one paragraph) and continue saying that we address the following challenges (four changes) - it would be great if we can give a name to each challange such as robustness, interpretability, etc. 5) Then go to our specific contributions.}
%Sec~\ref{sec2} introduces the background of the AC-OPF problem, Matpower and Scientific machine learning. Sec~\ref{sec3} presents the AC-OPF problem formulation. Then, we study the sensitivity of different features in Sec~\ref{sec4}, and the propose learning approach is outlined in Sec~\ref{sec5}.
%Sec~\ref{sec6} concludes the paper and presents several directions for future research.
%Conventional optimal power flow relies on the high computational cost of numerical optimization.
%
%In this paper, we propose to use neural networks to address this challenge.
%
%We first analyze the intermediate results during the original numerical optimization procedure(i.e., MIPS solver) and discover several critical variables that are most influential to the final outputs.
%
%Then, we study the sensitivity of input/output features and validate as the precision requirement of output variables.
%
%Third, we pre-process those variables and use a multi-task learning model to generate feasible solutions to given problems. 
%
%The multi-task learning model enables information sharing with related tasks and task-specific design for each output task.  
% we propose to adopt the generative network models for generating false solutions and use discriminative networks to tell whether a given solution is feasible or not.
%
%
%Extensive experimental results demonstrate that our method achieves comparable accuracy with the numerical optimization algorithms while making a significant reduction of computation costs.

% Power grid simulation aims to dispatch the generators according to given power requirements~\textcolor{wq}{??}.
% %
% The traditional powergrid simulation relies on numerical optimization and  suffers from high computational cost.
% %
% To this end, we introduce a multitask learning model to reduce the computation cost. 
% %
% In particular, we analyze the Lagrangian multipliers in the original numerical optimization procedure (i.e., the MIPS solver) and discover several critical multipliers that are most influential to the final simulation quality. 
% %
% Then, we study the sensitivity of the correctness of modeling output to the final simulation quality.  %and validate as the precision requirement of output variables.
% Third, we propose a multi-task learning model to generate a warm startpoint solution for the powergrid simulation. 
% %
% The multitask-based model allows the prediction of the startpoint solution as well as the Lagrangian multipliers to share knowledge, hence improves prediction accuracy substantially.


%The multi-task learning model enables information sharing with related tasks and task-specific design for each output parameters. 
%Extensive experimental results demonstrate that our method achieves comparable accuracy with the original numerical optimization algorithms while achieving $1.46\times$ speedup (in terms of execution time). 


%The Eulerian fluid simulation is an important HPC application. The neural network has been applied to accelerate it. The current methods that accelerate the fluid simulation with neural networks lack flexibility and generalization. In this paper, we tackle the above limitation and aim to enhance the applicability of neural networks in the Eulerian fluid simulation. We introduce Smart-fluidnet, a framework that automates model generation and application. Given an existing neural network as input, Smart-fluidnet generates multiple neural networks before the simulation to meet the execution time and simulation quality requirement. During the simulation, Smart-fluidnet dynamically switches the neural networks to make best efforts to reach the user’s requirement on simulation quality. Evaluating with 20,480 input problems, we show that Smart-fluidnet achieves 1.46x and 590x speedup comparing with a state-of-the-art neural network model and the original fluid simulation respectively on an NVIDIA Titan X Pascal GPU, while providing better simulation quality than the state-of-the-art model.

\begin{comment}
In this paper, we introduce a framework ``Smart-PGsim'' to address these challenges mentioned above. Smart-PGsim has three major components. (1) It includes a tool to perform sensitivity study. 
%
The sensitivity study includes component analysis and prior analysis for addressing the robustness and systematical design correspondingly.
%
We first quantify the sensitivity of related components with respect to simulation success rate and imposes the quantized sensitivity into the loss function for improving model robustness.
%
Our prior analysis refers to adopting a perturbed ground truth signal to trigger the warm-start of a AC-OPF solver.
%
After the component analysis, we conduct the \textit{prior analysis} to systematically guide the evolution of model topology.
%
(2) Smart-PGsim  enables information sharing and customizes specific designs for multiple tasks by a multitask learning model. 
The multitask model generate a warm-start point to initial AC-OPF solver, which guarantees the optimality of final solution. % 
(3) Smart-PGsim also impose physics constraints in loss function with transformed equality and inequality constraints from the original problem formulations. 
\end{comment}
%\textcolor{red}{Maybe we do not need to talk about this, because you have corresponding networks for each bus case.}
%
%\textcolor{red}{what's the difference between $P_d,Q_d$ and the four input variables? Did you mentioned it?}
%%\textcolor{gk}{how did we determine this percentage? empirically? is there any papers that we can give a reference?}%We draw two observations from Figure~\ref{fig:sec7_2}: (1) The outputs of Smart-fluidnet are closer to the target value than those of the Tompson's model; (2) The variances of Smart-fluidnet are smaller than those of Tompson's model.
%These two observations reveal that Smart-fluidnet can give more \textit{consistent simulation quality} than the Tompson's model, which is crucial for dealing with largely diversified input problems.%\textcolor{gk}{why with and without? the caption does not match with the description}} 
 %\textcolor{red}{put\ the\ denominator\ up}%\textcolor{gk}{I didn't understand what you mean by the previous sentence.}%\textcolor{gk}{1x speedup reads weird, what about just saying positive speedup?}% \begin{table}[!t]
% \centering
% \caption{ for the five problem sizes with/without physical constraints.
% }
% \vspace{-10pt}
% \label{tab:model_speedup}
% \begin{tabular}{l p{0.9cm}p{0.9cm}p{0.9cm}p{1.1cm}p{1.1cm}}
% \hline
% Problem size  & 14-bus & 30-bus & 57-bus & 118-bus & 300-bus \\
% \hline   
% Without Constraints & 100\% & 91.7\% &100\% &100\% & 80.5\%\\
% With Constraints & 1.38$\times$ & 1.16$\times$ & 1.35$\times$& 1.66$\times$& 1.91$\times$ \\
% \hline
% \end{tabular}
% \end{table}

%\textcolor{gk}{maybe it is better to say "solid line"} \textcolor{gk}{dashed line}
%(lines marked with ``solid line'' represents \name with physics constraints and lines marked with dashed line represents \name without physics constraints).%%offers lower training loss (i.e., higher prediction accuracy).%\textcolor{red}{BTW, where is the 2000 validation samples???}%\textcolor{gk}{could it be possible to change the legend in Figure 5 - rather than saying "no" maybe "without"}
% \begin{table}[!t]
% \centering

% \caption{Normalized success rate comparison for the five test systems with/without physical constraints.
% }
% \vspace{-10pt}
% \label{tab:model_distribution}
% \begin{tabular}{l p{0.9cm}p{0.9cm}p{0.9cm}p{1.1cm}p{1.1cm}}
% \hline
% Problem size  & 14-bus & 30-bus & 57-bus & 118-bus & 300-bus \\
% \hline   
% None constraints & 86.12\% & 82.16\% &79.43\% &74.60\% & 70.38\%\\
% With constraints & 50.56\% & 18.10\% & 11.12\%& 4.07\%& 16.15\% \\
% \hline
% \end{tabular}
% \end{table}
%\item Using 10,000 problems as the simulation input for evaluation and using the original AC-OPF simulation as a baseline, \name brings 49.2\% performance improvement on average (with the consideration of neural network modeling cost) \textcolor{gk}{maybe also "up to X-91 percentage"}. For all of the input problems, \name gives an initial solution that leads to the simulation convergence without losing the optimality of the \textcolor{gk}{is this solution refering to the final solution?} solution.% \\
% \\
% \textcolor{gk}{Does it make sense to replace the previois bullet with this? - Using 10,000 problems as the simulation input for evaluation and using the original AC-OPF simulation as a baseline, \name brings 49.2\% performance improvement on average (with the consideration of neural network modeling cost), up to 91\%, without losing the optimality of the final solution}
% \\
% \\
% \textcolor{gk}{also this 49 percentage refers to what? we use this number only abstract, intro an conclusion. I think it is table 3}%The equality constraints in Eqn.\ref{eq:1b} consists of $1 \times n_b$ nonlinear real and $1 \times n_b$ reactive power balance equations.%maybe need add equtaion in page 60
%\textcolor{gk}{I just wonder if we need to talk about Matpower under problem formulation. The MISP solver is one of the solvers used to solve the Newton linear system?}
%\textcolor{wq}{%this equality constrained problem \textcolor{red}{(which equality constrained problem? $H(X)+Z=0$?)} is as follows. 
%Matpower performs power grid simulation with the primal-dual interior-point solver called Matlab Interior Point Solver (MIPS). 
%To solve the AC-OPF problem, the solver converts the inequality constraints in Eqn.~(\ref{eq:1c}) into equality constraints using a barrier function and vector of positive slack variables $Z$, i.e., $H(X)+Z=0$. Given the value of $\gamma$, the Lagrangian for this equality constrained problem is


In Table~\ref{tab:pre-processing}, we show the results of using different pre-processing methods.
%
The speed-up for standardization against none pre-processing reaches 1.4918 at a 100\% success rate.
%
In contrast, the normalization has a slightly lower speed-up of 1.3929.
%
This demonstrates that standardization can eliminate the metric variance between different input features.
%
% TOO BAD explanation:
Although normalization has a similar effect, it may lose the intra-feature differences.
%
Consequently, our neural networks show better results with standardization techniques.


\begin{table}[!t]
  \begin{center}
    \caption{{Comparisons between different pre-processing methods.}}
    \label{tab:pre-processing}
    \begin{tabular}{l c r}
      \toprule % <-- Toprule here
      \textbf{Pre-processing} & \textbf{Speed up} & \textbf{Success Rate (\%)}\\
    %   $\alpha$ & $\beta$ & $\gamma$ \\
      \midrule % <-- Midrule here
      None & --- &  100.00 \\
      Normalization & 1.3929 & 100.00 \\
      Standardization & 1.4918 &  100.00 \\
      \bottomrule % <-- Bottomrule here
    \end{tabular}
  \end{center}
\end{table}


\section{Progress}
\subsection{Installation}
\textcolor{wq}{WQ: How to install matflow.}

\textcolor{wq}{Ting: How to install autokeras.}


The installation of Auto-Keras is the same as other python packages. Noting Auto-Keras currently is only compatible with: Python 3.6. The latest stable version can be installed by running the following pip installation command in your terminal: pip install autokeras

\subsection{Variable dependency}

\subsection{Model Training}

\subsection{Model topology morphsim}
\textcolor{wq}{Ting: 1-2pages. and add more subsections if you want.}

\subsection{}

\begin{comment}
List what is the current problem in ACOPF;

Existing works and their problems;

what our motivation? how we improve the problem?

\textcolor{wq}{follow these two papers:
1.learning warm-start points for AC optimal power flow;
2.DeepOPF: Deep Neural Network for DC optimal power flow;
}
\end{comment}
\begin{abstract}
Conventional optimal power flow relies on high computational cost of numerical optimization.
%
In this paper, we propose to use neural networks to address this challenge by providing an alternative to this problem.
%
We first analyze the intermediate results during the original numerical optimization procedures and discover several critical variables that are most influential to the final outputs.
%
Hence we propose to select those variables as feature inputs for composing our training samples.
%
Second, we pre-process those variables and use multi-task learning to generate feasible solutions to given problems. 
%
Third, we propose to adopt the generative network models for generating \textcolor{wq}{....,}  and use discriminative networks to tell whether a solution is feasible or not.
%
The discriminative network plays a role to help experts quickly decide whether a solution \textcolor{wq}{... }.
%
Extensive experimental results demonstrate that our method achieves comparable accuracy with the numerical optimization algorithms while achieving large reduction of computation costs.
\end{abstract}


We show the results of three types of models in Table~\ref{tab:model_effi}.
%
The model type \uppercase\expandafter{\romannumeral2} and  model type \uppercase\expandafter{\romannumeral3} obtain a higher speed up and better success rate than model type \uppercase\expandafter{\romannumeral1}, demonstrating the efficacy of using shared features.
Moreover,  model type \uppercase\expandafter{\romannumeral3} achieves better performance than  model type \uppercase\expandafter{\romannumeral2}, which shows the efficiency of tailored design of specific layers.

\begin{table}[!th]
  \begin{center}
    \caption{{Comparisons between different model types.}}
    \label{tab:model_effi}
    \begin{tabular}{l c r}
      \toprule % <-- Toprule here
      \textbf{Model type} & \textbf{Speed up} & \textbf{Success Rate (\%)}\\
    %   $\alpha$ & $\beta$ & $\gamma$ \\
      \midrule % <-- Midrule here
     % None & --- &  100.00 \\
      Model Type \uppercase\expandafter{\romannumeral1} & 1.2987  &  94.00 \\
      Model Type \uppercase\expandafter{\romannumeral2} & 1.4039  & 100.00 \\
     Model Type \uppercase\expandafter{\romannumeral3} & 1.4918  & 100.00 \\
      \bottomrule % <-- Bottomrule here
    \end{tabular}
  \end{center}
\end{table}


We also test model performance in larger Power-grid network sizes. In table \ref{tab:model_perf}, we observe that the \textcolor{wq}{.....}

\begin{table}[!th]
  \begin{center}
    \caption{{Model performance in different input sizes.}}
    \label{tab:model_perf}
    \begin{tabular}{l c r}
      \toprule % <-- Toprule here
      \textbf{Model type} & \textbf{Speed up} & \textbf{Success Rate (\%)}\\
    %   $\alpha$ & $\beta$ & $\gamma$ \\
      \midrule % <-- Midrule here
     % None & --- &  100.00 \\
      IEEE-30Bus & 1.4918   &  100.00 \\
      IEEE-118Bus & 1.6770  & 100.00 \\
     IEEE-300Bus& 2.0244 & 100.00 \\
      \bottomrule % <-- Bottomrule here
    \end{tabular}
  \end{center}
\end{table}

\begin{comment}
\begin{gather}
 \notag   \min_{X}[f(X)-\gamma\sum_{m=1}^{n_i}\ln(Z_m)]\\
s.t.\
  G(X)=0\\
 \notag   H(X)+Z=0\\
 \notag   Z>0  
 \end{gather}
\end{comment}


%By taking the partial derivatives with respect to each of the variables will yield:
%\begin{equation}
 %   L_X^{\gamma}(X,Z,\lambda,\mu)=f_X+\mathbf{\lambda}^\intercal\\G(X)+\mathbf{\mu}^\intercal\\H(X)
%\end{equation}
%\begin{equation}
%    L_Z^{\gamma}(X,Z,\lambda,\mu)=\mathbf{\mu}^\intercal\\-\gamma\mathbf{e}^\intercal\\\textbf{[Z]}^{-1}
%\end{equation}
%\begin{equation}
 %   L_Z^{\lambda}(X,Z,\lambda,\mu)=\mathbf{G}^\intercal\\(X)
%\end{equation}
%\begin{equation}
%    L_Z^{\mu}(X,Z,\lambda,\mu)=\mathbf{H}^\intercal\\(X)+\mathbf{Z}^\intercal
%\end{equation}
%The Hessian of the Lagrangian with respect to X is given by
%\begin{equation}
%    L_{XX}^{\gamma}(X,Z,\lambda,\mu)=f_{XX}+G_{XX}(\lambda)+H_{XX}(\mu).
%\end{equation}
%The first order optimality (Karush-Kuhn-Tucker) conditions for this problem are satisfied when the partial derivatives of the Lagrangian above are all set to zero:
%\begin{equation}
 %  \begin{split} F(X,&Z,\lambda,\mu)=0,\\
 %   &Z>0\\
 %   &\mu>0
 %   \end{split}
%\end{equation}
%with
%\begin{equation}
 %   F(X,Z,\lambda,\mu)=\begin{vmatrix}
%\mathbf{L_Z^{\lambda}}^\intercal\\
%[\mu]Z-\gamma e\\
%G(X)\\
%H(X)+Z\\
%\end{vmatrix}=\begin{vmatrix}
%\mathbf{f_X}^\intercal+\mathbf{G_X}^\intercal \lambda+\mathbf{H_X}^\intercal \lambda\\
%[\mu]Z-\mu e\\
%G(X)\\
%H(X)+Z\\
%\end{vmatrix}.
%\end{equation}


\begin{figure}[htbp]
\centering
\subfigure[pic1.]{
\includegraphics[width=6cm]{Figures/x_VA_Distribution.pdf}
%\caption{fig1}
}
\quad
\subfigure[pic2.]{
\includegraphics[width=6cm]{Figures/x_VM_Distribution.pdf}
}
\quad
\subfigure[pic3.]{
\includegraphics[width=6cm]{Figures/x_PG_Distribution.pdf}
}
\quad
\subfigure[pic4.]{
\includegraphics[width=6cm]{Figures/x_QG_Distribution.pdf}
}
\caption{ pics}
\end{figure}


\begin{figure}[htbp]
\centering
\subfigure[pic1.]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=5.5cm]{Figures/lam_Distribution.pdf}
%\caption{fig1}
\end{minipage}%
}%
\subfigure[pic2.]{
\begin{minipage}[t]{0.34\linewidth}
\centering
\includegraphics[width=5.5cm]{Figures/mu_Distribution.pdf}
%\caption{fig2}
\end{minipage}%
}%
\subfigure[pic3.]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=5.5cm]{Figures/z_Distribution.pdf}
%\caption{fig2}
\end{minipage}
}%

\centering
\caption{ pics}
\end{figure}

